C-GAIL: Stabilizing Generative Adversarial Imitation Learning with Control Theory

Generative Adversarial Imitation Learning (GAIL) trains a generative policy to mimic a demonstrator. It uses on-policy Reinforcement Learning (RL) to optimize a reward signal derived from a GAN-like discriminator. A major drawback of GAIL is its training instability - it inherits the complex training dynamics of GANs, and the distribution shift introduced by RL. This can cause oscillations during training, harming its sample efficiency and final policy performance. Recent work has shown that control theory can help with the convergence of a GAN's training. This paper extends this line of work, conducting a control-theoretic analysis of GAIL and deriving a novel controller that not only pushes GAIL to the desired equilibrium but also achieves asymptotic stability in a 'one-step' setting. Based on this, we propose a practical algorithm 'Controlled-GAIL' (C-GAIL). On MuJoCo tasks, our controlled variant is able to speed up the rate of convergence, reduce the range of oscillation and match the expert's distribution more closely both for vanilla GAIL and GAIL-DAC.

==> Styles/input/1-introduction.tex <==

% \begin{table}[hb] 
%     \centering
%     \begin{tabular}{|c|c|c|c|c|} 
%     \hline
%            & Empirical work & Converge & Asymptotically converge \\
%     \hline
%       GAIL \cite{ho2016generative}  & \checkmark & & \\
%       AIRL \cite{fu2017learning}     & \checkmark & & \\
%       GAIL + BC \cite{jena2021augmenting} & \checkmark & & \\
%       WAIL \cite{xiao2019wasserstein} & \checkmark & & \\ 
%       DAC \cite{kostrikov2018discriminator} & \checkmark & & \\
%       f-MAX \cite{ghasemipour2020divergence} & & \checkmark & \\
%       \citet{chen2020computation} & & \checkmark & \\
%       \citet{zhang2020generative} & & \checkmark & \\
%       \citet{guan2021will} & & \checkmark & \\
%     \hline
%       Ours & & & \checkmark \\
%     \hline
%     \end{tabular}
%     \caption{Stability guarantee for different GAIL variants under one-step setting.  The assumptions regarding the MDP and reward function for \cite{chen2020computation, zhang2020generative, guan2021will} are explicitly listed in Section \ref{relatedwork}. In comparison, our method does not require such assumptions and achieves better convergence guarantee. 1. linear model; 2. strongly concave objective; 3. converge to local; 4. converge to global. 5. empirical. 6. theoretical. 7. type 1. 8. type 2.}
%     \label{comparework}
% \end{table}



\section{Introduction}
Generative Adversarial Imitation Learning (GAIL) \citep{ho2016generative} aims to learn a decision-making policy in a sequential environment by imitating trajectories collected from an expert demonstrator. 
Inspired by Generative Adversarial Networks (GANs) \citep{goodfellow2014generative}, GAIL consists of a learned policy serving as the generator, and a discriminator  distinguishing expert trajectories from the generated ones. 
% alternating between training a discriminator to differentiate between expert and generated actions and a generative policy that aims to deceive this discriminator. 
% This method, leveraging the robust framework of GANs, offers distinct advantages over other imitation learning strategies such as Inverse Reinforcement Learning (IRL) or Behavior Cloning (BC), primarily due to blabla reason.
The learned policy is optimized by Reinforcement Learning (RL) algorithms with a reward signal derived from the discriminator.
% \jianfei{it is weird that anything can be optimized by ``RL''. I think RL is an area, a paradigm, a problem, rather than an optimizer.}
This paradigm offers distinct advantages over other imitation learning strategies such as Inverse Reinforcement Learning (IRL), which requires an explicit model of the reward function \citep{ng2000algorithms}, and Behavior Cloning (BC), which suffers from a distribution mismatch during roll-outs \citep{codevilla2019exploring}. 
% However, GAIL does bring certain challenges. One key issue it inherits from GANs is instability during training \citep{mescheder2018training}. \jianfei{what does it mean by ``unstable''? This is important, since RL people seem to have different understanding to this. They think unstable means you repeat the algorithm with different random seeds, the performance numbers have large variations.} This problem, while theoretically manageable in linear settings or strongly concave objective function \citep{zhang2020generative, guan2021will}, manifests in practice as oscillating training curves and an inconsistency in matching the expert's performance. 

Meanwhile, GAIL does bring certain challenges. One key issue it inherits from GANs is \emph{instability} during training \citep{mescheder2018training}. GAIL produces a difficult minimax optimization problem, where the convergence of the discriminator and the policy generator towards their optimal points is not guaranteed in general. 
This problem manifests in practice as oscillating training curves and an inconsistency in matching the expert's performance (Fig.~\ref{fig:dac-return}). However, current empirical works \citep{fu2017learning, jena2021augmenting, xiao2019wasserstein, kostrikov2018discriminator, swamy2022minimax} of GAIL mostly focus on improving the sample efficiency and final return for learned policy, which do not resolve our problem of unstable training. On the other hand, existing theoretical works \citep{chen2020computation,cai2019global, zhang2020generative, guan2021will} on GAIL's convergence are based on strong assumptions and do not yield a practical algorithm to stabilize training. 

% to the optimal . 
% Specifically, during its training process, the discriminator and the policy generator rarely converge to their optimal points. 

% works studying GAIL \citep{chen2020computation, cai2019global, zhang2020generative, guan2021will} have two limitations: they either make strong assumptions, or only assure convergence to a local instead of global optimum. For instance, \citet{cai2019global} and \citet{zhang2020generative} require i.i.d. samples and the MDP be linear to assure convergence to a global optimum, and \citet{guan2021will} assume the objective function to be strongly concave. 
% Meanwhile, \citet{chen2020computation} study only local convergence.
% \tp{I'd keep this detail in 1.1}
% In summary, the convergence behavior of GAIL under general assumptions is unclear and this motivates our goal: \textbf{Can GAIL converge to the global optimum in the general case?}


% Existing theoretical work studying GAIL \tp{GAIL or GANs?} \citep{chen2020computation, cai2019global, zhang2020generative, guan2021will} has two limitations: they either make strong assumptions, or only assure convergence to a local instead of global optimum (Table\ref{comparework}). For instance, \citet{chen2020computation} only guarantee GAIL to converge, not necessary to our global optimal. \citet{cai2019global} and \citet{zhang2020generative} require i.i.d. samples and linear MDP to converge to global optimal. \citet{guan2021will} assume the objective function to be strongly concave to reach the global optimal. However, the convergence behavior of GAIL under general setting is unclear and this motivates our goal:

%Existing theoretical works studying GAIL \citep{chen2020computation, cai2019global, zhang2020generative, guan2021will} have two limitations: they either make strong assumptions, or only assure convergence to a local instead of global optimum. For instance, \citet{cai2019global} and \citet{zhang2020generative} require i.i.d. samples and the MDP be linear to assure convergence to a global optimum, and \citet{guan2021will} assume the objective function to be strongly concave. 
%Meanwhile, \citet{chen2020computation} study only local convergence.
% \tp{I'd keep this detail in 1.1}
% In summary, the convergence behavior of GAIL under general assumptions is unclear and this motivates our goal: \textbf{Can GAIL converge to the global optimum in the general case?}
% \makebox[\textwidth]{
%      \textit{Can GAIL converge to global optimal under general setting? } }
% Existing theoretical work has two limitations: 1. strong assumptions: linear MDP. 2. converge is not what we want, we want it to converge to the expert policy (stability). 

In this paper, we study GAIL's training stability using control theory. We describe how the generative policy and discriminator evolve over training at timestep $t$ with a dynamical system of differential equations. We study whether the system can converge to the \emph{desired state}  where the generator perfectly matches with the expert policy and the discriminator cannot distinguish generated from expert trajectories. This surprisingly reveals that the desirable state is not a equilibrium of the system, indicating that existing algorithms do not converge to the expert policy, even with unlimited data and model capacity.
In response, we study a ``one-step GAIL'' setting, and design a controller that does create an equilibrium at the desired state. We theoretically prove that this controller achieves \textit{asymptotic stability} around this desired state, which means that if initialized within a sufficiently close radius, the generator and discriminator will indeed converge to it.

%{Drawing on recent advancements studying GANs with control theory \citep{xu2020understanding, luo2023stabilizing}, this paper shows that indeed GAIL \textit{can} be made to converge to the global optimum and reach asymptotic stability.  We provide the first analysis of GAIL as a dynamical system from the perspective of control theory (Section \ref{sec:dynamic}). 



Motivated by our theoretical analysis, we propose C-GAIL, which incorporates a pragmatic controller that can be added as a regularization term to the loss function to stabilize training in practice. 
Empirically we find that our method speeds up the convergence, reduces the range of oscillation in the return curves (shown on Fig. \ref{fig:dac-return}), and matches the expert's distribution more closely on GAIL-DAC and other imitation learning methods for a suite of MuJoCo control tasks.


% \tp{I'm wary of these claims about global convergence in the general setting (general wrt what?). Do we really provide this guarantee? I thought we only show that: 1) the desired state is an equilibrium (whether this is a global minimum I'm not sure, it seems possible that there are other states with lower losses?). 2) if we intialize within a radius of delta around this equialibrium, we will converge to it (asymptotic stability), but we're not guaranteed to converge to that point if we initialize outside that radius. How do we know if we are inside that radius? I'm also not clear on what assumptions we make to get this asymptotic stability -- infinitely small step size?}

% \tp{in general I worry this is too much detail too early. Is the point of this to set it up immediately as a theoretical paper? I might be tempted to revert to the ICML intro and modify from there.}

% \junz{fig.1 was not referred in Intro while putting it in the front?}
% This paper improves the stability and convergence properties of GAIL by drawing on recent advancements studying GANs with control theory \citep{xu2020understanding, luo2023stabilizing}.  We provide the first analysis of GAIL as a dynamical system from the perspective of control theory (Section \ref{sec:dynamic}). This surprisingly reveals that the desirable minimax point is not an equilibrium of GAIL. In response, we propose a "one-step GAIL" setting, and design a controller that does create an equilibrium at the desired point (Section \ref{control}). We theoretically prove that this controller allows the dynamical system of GAIL's training to achieve \textit{asymptotic stability}. Motivated by this, we propose C-GAIL, which incorporates a pragmatic controller that can be added as a regularization term to the loss function in practice.  Empirically we find that our method speeds up the convergence rate and reduces the range of oscillation in the return curves, and matches the expert's distribution more closely on GAIL-DAC and other imitation learning methods for a suite of MuJoCo control tasks (Section \ref{Evaluation}).

% Concretely, we \tj{compare our method to existing works in table \ref{comparework}} and offer several contributions.\jianfei{under polished} 
% \begin{itemize}
% % \item Study the training process of GAIL as dynamical system
% \item We provide the first analysis of GAIL as a dynamical system from the perspective of control theory.
% \item We identify an issue with convergence of GAIL, showing that the desired state is not an equilibrium point.
% \item We propose a simplified "one-step GAIL" model, where we design a controller that we theoretically prove is \textit{asymptotically stable}.
% \item Based on this ideal controller, we propose a practical objective function for the discriminator, resulting in our C-GAIL algorithm. 
% % This is on GAIL-DAC and vanilla GAIL.
% % \item Design a controller to alter GAIL's training dynamic and push it to the desired equilibrium and theoretically prove that our controlled GAIL achieves \textit{asymptotic stability}
% \item Empirically we find that our method speeds up the convergence rate and reduces the range of oscillation in the return curves, and matches the expert's distribution more closely on GAIL-DAC. 
    
% \end{itemize}



% \vspace{1in}
% \tp{original version.}
% Generative Adversarial Imitation Learning (GAIL) \citep{ho2016generative} is an effective method to learn sequential decision-making policies such as controlling autonomous vehicles or robots \citep{choi2021trajgail, bhattacharyya2022modeling}, modeling real-life agents \citep{song2018multi}, and even text generation \citep{muthukumar2021generative}. GAIL is an imitation learning (IL) method, which is a class of methods that includes behavioral cloning (BC) \citep{pomerleau1991efficient, esmaili1995behavioural} and inverse reinforcement learning (IRL) \citep{ng2000algorithms, abbeel2004apprenticeship, hadfield2016cooperative}. Despite its straightforward implementation, BC suffers from accumulating distribution shifts \citep{codevilla2019exploring} as a supervised learning algorithm. On the other hand, IRL requires high computational costs for bi-level optimization since it searches for the optimal reward function in the outer loop and explicitly solves the RL subproblem in the inner loop. Even though \citet{ziebart2008maximum} employs the max entropy IRL to improve the efficiency of IRL, the optimal reward function of IRL may not be unique. To resolve the issues of IRL, GAIL combines IRL with generative adversarial networks (GANs) \citep{goodfellow2014generative} and solves the inner-loop RL problem via minimax optimization. Given expert trajectories $\tau_E$ sampled from expert policy $\pi_E$, GAIL alternatively trains a policy generator $\pi$ and a discriminator $D$, and ultimately, the policy generator approaches the expert policy, and the discriminator becomes indistinguishable for the expert policy and generated policy. Similar to GANs, the training process of GAIL can be formulated as a minimax optimization problem, where the policy generator and the discriminator compete with each other in order to reach equilibrium. 

% Unfortunately, GAIL inherits the notorious and well-known issue of GANs--unstable in training \citep{mescheder2018training, luo2023stabilizing}. While some theoretical work suggests that GAIL can attain global convergence under linear settings \citep{zhang2020generative, guan2021will}, empirically, it is well observed that GAIL has oscillating training curves and is unable to approach expert policy. In this paper, we 

% \begin{itemize}
% \item Transform the training process of GAIL into a system of differential equations to represent the dynamic of the policy generator and the discriminator.
% \item Formally identify the issue that GAIL exhibits unstable training behaviors and cannot converge to the minimax equilibrium as desired by transforming GAIL proving its incompetence to reach optimal points.
% \item Design a controller to alter GAIL's training dynamic and push it to the desired equilibrium and theoretically prove that our controlled GAIL achieves \textit{asymptotic stability}
% \item Speed up the convergence speed and reduce the range of oscillation in terms of the return compared to GAIL-DAC and original GAIL
    
% \end{itemize}

\begin{figure}[t!]
\centering
\begin{minipage}{0.327\linewidth}
	\centering
        {\footnotesize Half-Cheetah} 
	\includegraphics[width=\linewidth]{input/fig/Half-Cheetah4ExpertDemostrations.pdf}
\end{minipage} 
\begin{minipage}{0.327\linewidth}
	\centering
 {\footnotesize Walker2d}
	\includegraphics[width=\linewidth]{input/fig/Walker2d4ExpertDemostrations.pdf}
\end{minipage} 
\begin{minipage}{0.327\linewidth}
	\centering
 {\footnotesize Reacher}
	\includegraphics[width=\linewidth]{input/fig/Reacher4ExpertDemostrations.pdf}
\end{minipage} \\


\begin{minipage}{0.327\linewidth}
	\centering
  {\footnotesize Ant}
	\includegraphics[width=\linewidth]{input/fig/Ant4ExpertDemostrations.pdf}
\end{minipage} 
\begin{minipage}{0.327\linewidth}
	\centering
  {\footnotesize Hopper}
	\includegraphics[width=\linewidth]{input/fig/Hopper4ExpertDemonstrations.pdf}
\end{minipage} 
 \\

  \caption{Normalized return curves for controlled GAIL-DAC with four expert demonstrations on five MuJoCo environments averaged over five random seeds. The x-axis represents the number of gradient step updates in millions and the y-axis represents the normalized environment reward, where 1 stands for the expert policy return and 0 stands for the random policy return
  % \jianfei{font size is too small. lots of blanks} \tj{tried to delete the blanks and increase the font for title. The text for legends and x, y labels does not fit for a larger font.}
  }
    \label{fig:dac-return}
    \vspace{-0.1in}
\end{figure}




\subsection{Related Work} \label{relatedwork}
% Previous works have been done to improve the performance of GAIL in terms of sample efficiency and robustness in different environments. While GAIL utilizes Jensen-Shannon (JS) divergence to measure the similarity between state-action pair distribution,  \citet{zhang2020f} replaces it with the f-divergence \citep{ghasemipour2020divergence} for higher data efficiency. \citet{kostrikov2018discriminator} uses a discriminator-actor-critic (DAC) to improve the sample efficiency of GAIL and reduce the bias for the reward function. \citet{fu2017learning} present adversarial inverse reinforcement learning (AIRL) that designs a different discriminator based on GAIL to represent the reward function of IRL so that its reward function is more robust to variations in environments. \citet{wang2017robust} combine variational autoencoder (VAE) on demonstration trajectories to improve the robustness and avoid mode collapse. 
    

% \textbf{Convergence of GAIL}
% Some theoretical works are conducted for the stability analysis of GAIL. \citet{syed2008apprenticeship} analyze the convergence and stability of apprenticeship learning. \citet{chen2020computation} show that GAIL approaches a stationary point (may not be the optimal solution) with the gradient-based algorithm on general MDP and general reward function. \citet{zhang2020generative} introduces a natural policy gradient (NPG) algorithm and claims to achieve sublinear convergence to the global optimal solution. However, this work has restrictive theoretical assumptions on linear MDP and linear reward function, which are not applicable to real-life environments.    \citet{guan2021will} extend the convergence analysis to nonlinear MDP and nonlinear reward function. However, its convergence guarantee is under the assumption that the objective function is strongly concave. Both works of \citet{zhang2020generative} and \citet{guan2021will} lack empirical evidence to show that GAIL converges as claimed.  

% \textbf{Stability Analysis with Control Theory} In GANs, many stabilizing methods are proposed with control theory. \citet{xu2020understanding} propose a linear controller and locally stabilizes GANs. \citet{luo2023stabilizing} utilize Brownian motion controller and globally exponentially stabilize GANs. Both works analyze the stability of GANs' training with respect to the GANs' dynamic functions. However, rather than the expectation over the data distribution for GANs, the expectation over a policy in GAIL involves a Markov process, so the dynamic function for GANs is different from the one for GAIL, thus the controllers from \citet{xu2020understanding, luo2023stabilizing} for GANs are unable to apply on GAIL.


\textbf{Adversarial imitation learning.}
Inspired by GANs and inverse RL, Adversarial Imitation Learning (AIL) has emerged as a popular technique to learn from demonstrations.
% \citep{orsini2021matters}.
GAIL~\citep{ho2016generative} formulated the problem as matching an occupancy measure under the maximum entropy RL framework, with a discriminator providing the policy reward signal, bypassing the need to recover the expert's reward function. Several advancements were subsequently proposed to enhance performance and stability.
% ~\citep{baram2017end, fu2017learning, kostrikov2018dSiscriminator, kostrikov2020image, ghasemipour2020divergence, orsini2021matters}.
For instance, AIRL~\citep{fu2017learning} replaced the Shannon-Jensen divergence of GAIL by KL divergence.
\citet{baram2017end} explored combining GAIL with model-based reinforcement learning.
DAC~\citep{kostrikov2018discriminator} utilized a replay buffer to remove the need for importance sampling and address the issue of absorbing states.
Other empirical works such as \citep{jena2021augmenting, xiao2019wasserstein, kostrikov2018discriminator, swamy2022minimax, rajaraman2020toward} have been done to improve the sample efficiency and final return of GAIL. In contrast, our work focuses on the orthogonal direction of training stability. 
%\jianfei{No empirical work for improving training stability.}
% ~\citep{chen2020computation, zhang2020generative, guan2021will}.

Meanwhile, the convergence behaviors of AIL have also been investigated theoretically.
%from more of a theoretical standpoint to analyze the necessary conditions to converge.  
\citet{chen2020computation} proved that GAIL convergences to a stationary point (not necessarily the desired state). 
The convergence to the desired state has only been established under strong assumptions such as  i.i.d. samples and linear MDP \cite{cai2019global,zhang2020generative} and strongly concave objective functions \cite{guan2021will}. However, existing theory has not analyzed the convergence behavior to the desired state in a general setting, and has so far not presented practically useful algorithms to improve GAIL's convergence.
Our analysis in Sec.~\ref{sec:notconverge} show that GAIL actually \emph{cannot} converge to the desired state under general settings. Additionally, our proposed controller achieves not only a theoretical convergence guarantee, but also empirical improvements in terms of convergence speed and range of oscillation.
%empirical improvements by significantly 

% \citet{cai2019global} and \citet{zhang2020generative} proved 
% require i.i.d. samples and linear MDP to converge to global optimal. \citet{guan2021will} assume the objective function to be strongly concave to reach the global optimal. However, the convergence behavior of GAIL under general setting is unclear and this motivates our goal:



% showed that GAIL approaches a stationary point (though this may not be the optimal solution) with a gradient-based algorithm in a general Markov Decision Process (MDP). \citet{zhang2020generative} introduced a natural policy gradient (NPG) algorithm, showing it converges, sub-linearly, to the global optimum. \citet{guan2021will} extended the convergence analysis to non-linear MDPs with strongly concave objective function.
% In comparison, we work under general MDP and general reward function, and achieve asymptotically stable with a smaller radius of convergence.
% By contrast, our work begins from the novel perspective of dynamical systems, applied to the MDP setting, and is asymptotically stable with a smaller radius of convergence.  By contrast, our work analyzes GAIL under general MDP and objective function and begins from the novel perspective of dynamical systems. Moreover, we are the first work to reduce the radius of convergence for GAIL's training process and achieve asymptotically stability.


% However, they do not provide insights regarding speeding up the rate of convergence  and improve the stability for the training process of GAIL. 


% Existing theoretical work studying GAIL \tp{GAIL or GANs?} \citep{chen2020computation, cai2019global, zhang2020generative, guan2021will} has two limitations: they either make strong assumptions, or only assure convergence to a local instead of global optimum (Table\ref{comparework}). For instance, \citet{chen2020computation} only guarantee GAIL to converge, not necessary to our global optimal. \citet{cai2019global} and \citet{zhang2020generative} require i.i.d. samples and linear MDP to converge to global optimal. \citet{guan2021will} assume the objective function to be strongly concave to reach the global optimal. However, the convergence behavior of GAIL under general setting is unclear and this motivates our goal:



% Our work considers general MDPs and reward functions, and our proposed method is asymptotically stable with a smaller radius of convergence. \tp{need to be clearer about our contributions relative to this work. smaller compared to who? why is general better than non-linear?}

% \tj{Smaller compared to DAC and naive GAIL, Chen, Zhang, Guan's work are theoretical and they do not have experiment to compare with}
% \\ \tp{also is it necessary to list separately the MDP and reward fn? Isn't the reward function part of the MDP?}
% \tj{Yes reward function is a component of MDP, I'm following the related work previous work which separated list those two, we can combine them if you wish}
% \jianfei{I suppose we are doing an orthogonal direction with these works. We do not need to claim that our controlled-GAIL is better than all GAIL variants.}

% Adversarial Imitation Learning (AIL) proposes a maximum entropy occupancy measure matching method to recover the underlying policy by estimating and maximizing the underlying reward function, and becomes a key focus of the imitation learning field. 
% GAIL~\citep{ho2016generative} introduces a maximum entropy occupancy measure matching method and learns a discriminator to bypass the need for recovering the expert's reward function. Subsequently with GAIL, several advancements  have significantly enhanced practical performance and stability ~\citep{baram2017end, fu2017learning, kostrikov2018dSiscriminator, kostrikov2020image, ghasemipour2020divergence}.
% AIRL~\citep{fu2017learning} replaces the Shannon-Jensen divergence of GAIL by KL divergence.
% \citep{baram2017end} effectively integrates the GAIL framework with the principles of model-based reinforcement learning, creating a link between these two methodologies.
% DAC~\citep{kostrikov2018discriminator} utilizes a replay buffer that bypasses the need for importance sampling and addresses the issue of absorbing states.
% On the other hand, some theoretical works are conducted for the stability analysis of AIL~\citep{chen2020computation, zhang2020generative, guan2021will}.
% \citet{chen2020computation} shows that GAIL approaches a stationary point (may not be the optimal solution) with the gradient-based algorithm on general MDP and general reward function. \citet{zhang2020generative} introduces a natural policy gradient (NPG) algorithm and achieves sublinear convergence to the global optimal solution. \citet{guan2021will} extend the convergence analysis to nonlinear MDP and nonlinear reward function. In comparison, we work under general MDP and general reward function, and achieve asymptotically stable with a smaller radius of convergence.


\textbf{Control theory in GANs.} 
Control theory has recently emerged as a promising technique for studying the convergence of GANs.
\citet{xu2020understanding} designed a linear controller which offers GANs local stability. 
\citet{luo2023stabilizing} utilized a Brownian motion controller which was shown to offer GANs global exponential stability. 
%Both works analyze the stability of GANs' training with respect to their induced dynamical systems under linear simplified Dirac-GANs setting, and they extend the designed controllers from Dirac-GANs to normal GANs. 
However, for GAIL, the policy generator involves an MDP transition, which results in a much more complicated dynamical system induced by a policy acting in an MDP rather than a static data generating distribution. 
Prior theoretical analysis and controllers are therefore inapplicable. We  adopt different analysis and controlling techniques, to present new stability guarantee, controller, and theoretical results for the different dynamical system of GAIL. 

%Our work adopts this control theoretic perspective in a new setting -- we must deal with both a non-linear dynamical system, and an induced distribution of a policy acting in an MDP rather than a static data generating distribution. 
% rather than under a static data distribution of supervised learning, we consider the induced distribution of a policy acting in an MDP (and at times a simplified version of this).
% \tj{I added a sentence here}
% \tp{we more or less ignore the MDP aspect of the problem though. I might leave this a little vaguer.}

% rather than the expectation over the data distribution for GANs, the expectation over a policy in GAIL involves a Markov process, so the dynamic function for GANs is different from the one for GAIL, thus the controllers from \citet{xu2020understanding, luo2023stabilizing} for GANs are unable to apply on GAIL.

% \textbf{Control Theory on Adversarial Learning.} 
% Various methods for stabilization have been proposed under the principles of control theory.
% \citet{xu2020understanding} designs a linear controller and locally stabilizes GANs. 
% \citet{luo2023stabilizing} utilizes Brownian motion controller and globally exponentially stabilize GANs. Both works analyze the stability of GANs' training with respect to the GANs' dynamic functions. 
% However, rather than the expectation over the data distribution for GANs, the expectation over a policy in GAIL involves a Markov process, so the dynamic function for GANs is different from the one for GAIL, thus the controllers from \citet{xu2020understanding, luo2023stabilizing} for GANs are unable to apply on GAIL.


\iffalse
\begin{table}[ht] 
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|} 
    \hline
    & \multicolumn{3}{|c|}{Assumptions}&\multicolumn{2}{|c|}{Result}\\
    \hline
           &general&general& general  & converge to  & converge to \\
           & samples& MDP&  objective & local optimal &  global optimal\\
    \hline
      \citet{chen2020computation} &\cmark &\cmark &\cmark& \cmark & \xmark\\
      \citet{cai2019global}&\xmark &\xmark& \cmark&\cmark & \cmark  \\
      \citet{zhang2020generative} &\xmark&\cmark & \cmark &\cmark& \cmark \\
      \citet{guan2021will} &\cmark& \cmark& \xmark &\cmark & \cmark \\
    \hline
      Ours &\cmark &\cmark &\cmark&\cmark & \cmark \\
    \hline
    \end{tabular}
    \caption{Comparison of stability guarantee for theoretical GAIL variants. The assumptions regarding the MDP and reward function for \cite{chen2020computation, zhang2020generative, guan2021will} are explicitly listed in Section \ref{relatedwork}. In comparison, our method does not require above assumptions and achieves better convergence guarantee under 'one-step' setting. \jianfei{is the claim too strong? we still make quite strong assumptions.}
    % 1. linear model; 2. strongly concave objective; 3. converge to local; 4. converge to global. 5. empirical. 6. theoretical. 7. type 1. 8. type 2.
    }
    \label{comparework}
\end{table}
\fi



==> Styles/input/2-preliminary.tex <==

\section{Preliminaries}  \label{preliminary}
We start by formally introducing our problem setting, as well as necessary definitions and theorems relating to the stability of dynamical systems represented by Ordinary Differential Equations (ODEs).
% We first define the concepts of equilibrium and stability for a dynamical system. Then, we present the related theorem in control theory for the criteria of a stable dynamical system.

% In this section, we present our problem setting along with definitions and theorems on stability analysis for a dynamical system in the form of Ordinary Differential Equations (ODE). We first define the concepts of equilibrium and stability for a dynamical system. Then, we present the related theorem in control theory for the criteria of a stable dynamical system.

\subsection{Problem Setting} \label{setting}
Consider a Markov Decision Process (MDP), described by the tuple $\langle \mathcal{S}, \mathcal{A}, \mathcal{P}, r, p_0, \gamma \rangle$, where $\mathcal{S}$ is the state space, $\mathcal{A}$ is the action space, $\mathcal{P}(s'|s, a)$ is the transition probability function, $r(s, a)$ is the reward function, $p_0$ is the probability distribution of the initial state $s_0$, and $\gamma \in [0,1]$ is the discount factor. 
We work on the $\gamma$-discounted infinite horizon setting, and define the expectation with respect to a policy $\pi \in \Pi$ as the (discounted) expectation over the trajectory it generates. For some arbitrary function $g$ we have $\mathbb{E}_\pi[g(s, a)] \triangleq \mathbb{E}[\Sigma_{n=0}^\infty \gamma^n g(s_n,a_n)] $, where $a_n \sim \pi(a_n | s_n)$, $s_0 \sim p_0$, $s_{n+1} \sim \mathcal{P}(s_{n+1} | {s_n, a_n})$. 
Note that we use $n$ to represent the \textbf{environment timestep}, reserving $t$ to denote the \textbf{training timestep} of GAIL. For a policy $\pi \in \Pi$, We define its (unnormalized) state occupancy $\rho_{\pi}(s) =  \sum_{n=0}^{\infty} \gamma^n P(s_n=s|\pi)$. We denote $Q^{\pi}(s, a) = \mathbb{E}_{\pi}[\log D(\bar{s},\bar{a}) + \lambda \log \pi(\bar{a}|\bar{s})| s_0 = s, a_0 = a]$ and the advantage function $A^{\pi}(s,a)= Q^{\pi}(s,a) - \mathbb{E}_{\pi}[Q^{\pi}(s,a)]$. We assume the setting where we are given a dataset of trajectories $\tau_E$ consisting of state-action tuples, collected from an expert policy $\pi_E$. We assume access to interact in the environment in order to learn a policy $\pi$, but do not make use of any external reward signal (except during evaluation).


% Consider a Markov Decision Process (MDP), described by a tuple $\langle \mathcal{S}, \mathcal{A}, \mathcal{P}, r, p_0, \gamma \rangle$, where $\mathcal{S}$ is the state space, $\mathcal{A}$ is the action space, $\mathcal{P}(s'|s, a)$ is the transition probability function, $r(s, a)$ is the reward function, $p_0$ is the probability distribution of the initial state $s_0$, and $\gamma \in [0,1]$ is the discount factor. We work on the $\gamma$-discounted infinite horizon setting, and we define the expectation with respect to a policy $\pi \in \Pi$ to represent the expectation on the trajectory it generates: $\mathbb{E}_\pi[c(s, a)] \triangleq \mathbb{E}[\Sigma_{n=0}^\infty \gamma^n c(s_n,a_n)] $, where $a_n \sim \pi(a_n | s_n)$, $s_0 \sim p_0$, $s_{n+1} \sim \mathcal{P}(s_{n+1} | {s_n, a_n})$, and $c$ is any arbitrary function. Notice that here we intentionally use $n$ to represent the agent time step to avoid confusion with the training time $t$ of the generative adversarial imitation learning later. For a policy $\pi \in \Pi$, We define its occupancy measure $\rho_\pi : \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}$ as $\rho_\pi(s,a) = \pi(a|s) \Sigma_{n=0}^\infty \gamma^n P (s_n = s | \pi)$. In practice, we are given trajectories $\tau_E$ from an expert policy $\pi_E$, and we want to learn our policy generator $\pi$.


% \subsection{Convergence of a dynamical system}
\subsection{Dynamical Systems and Control Theory}\label{sec:dynamical-systems}


% Suppose we have a dynamical system of ODE with initial value $x(0) = x_0$:
In this paper, we consider dynamical systems represented by an ODE of the form
\begin{equation}
    \frac{d x(t)}{dt} = f(x(t)) \label{dynamic_system},
\end{equation}
where $x$ represents some property of the system, $t$ refers to the timestep of the system and $f$ is a function.
% One important question in dynamical systems, is whether the solution trajectory $\{x(t)\}_{t\geq0}$ converges to some steady state value.
The necessary condition for a solution trajectory $\{x(t)\}_{t\geq0}$ converging to some steady state value is the existence of an `equilibrium'.
% \jianfei{use `quote' or ``quote'' for quotes}
% When considering the convergence behavior of a dynamical system (\ref{dynamic_system})\jianfei{use (\ref{dynamic_system})}, we first need to make sure such an equilibrium exists, which is a necessary condition for the system to converge.
\begin{definition} \label{eqdef} \textbf{(Equilibrium)} \citep{ince1956ordinary}
    A point $\Bar{x}$ is an \textit{equilibrium} of system (\ref{dynamic_system}) if $f(\Bar{x}) = 0$. Such an equilibrium is also called a \textit{fixed point}, \textit{critical point}, or \textit{steady state}.
\end{definition}
\vspace{-0.05in}
Note that a dynamical system is unable to converge if
    an equilibrium does not exist.
%
% \begin{definition} \label{eqdef} \textbf{(Equilibrium)} \citep{ince1956ordinary}
%     A point $\Bar{x}$ is an \textit{equilibrium} of system (\ref{dynamic_system}) if $f(\Bar{x}) = 0$. Such an equilibrium is also called a \textit{fixed point}, \textit{critical point}, or \textit{steady state}.
% \end{definition}
% When we are considering the convergence behavior of a dynamical system (\ref{dynamic_system})\jianfei{use (\ref{dynamic_system})}, we first need to make sure such an equilibrium exists, which is a necessary condition for a dynamical system to converge. 
% \begin{remark} \label{convergeremark}
%    A dynamical system is unable to converge if
%     an equilibrium does not exist.
% \end{remark}
%
%
% \subsection{Stabilizing dynamical system with Control Theory}
% The field of control theory has studied how to drive dynamical systems to desired states. This can be achieved through the addition of a `controller' to allow influence over the dynamical system's evolution, for example creating an equilibrium at some desired state, and encouraging convergence to that equilibrium.
% % leading to convergence at a desired equilibrium.
% % In control theory, a controller can be added into a dynamical system to alter its solution trajectory. 
% % In control theory, a controller can be added into a dynamical system to alter its solution trajectory. Given a dynamical system that does not converge, a controller can be designed to push the dynamic to the required equilibrium and improve the stability of this dynamical system. 
% \begin{definition} \textbf{(Controller)} \citep{brogan1991modern}
%     A \textit{controller} of a dynamical system is a function $u(t)$ such that
%     \begin{equation}
%         \frac{d x(t)}{dt} = f(x(t)) +u(t) \label{dynamic_control} .
%     \end{equation}
% \end{definition}
% Given a dynamical system that does not converge, a controller can be designed to push the dynamic to the required equilibrium and improve the stability of this dynamical system. 
%
A second important property of dynamical systems is `stability'. The stability of a dynamical system can be described with Lyapunov stability criteria. More formally, suppose $\{x(t)\}_{t \geq 0}$ is a solution trajectory of the above system (\ref{dynamic_system}) with equilibrium $\Bar{x}$, we define two types of stability. 
% \tp{any reason for pointing to (2)? I think it equally refers to (1)?} \tj{TODO}
% We define two types of stability: Lyapunov stability and asymptotic stability. 



\begin{definition} \label{def_stable_lyapunov}
\textbf{(Lyapunov Stability)} \citep{glendinning1994stability}
System (\ref{dynamic_system}) is \textit{Lyapunov Stable} if given any $\epsilon > 0$, there exists a $\delta > 0$ such that whenever $\lVert x(0) - \Bar{x} \rVert \leq \delta$, we have $\lVert x(t) - \Bar{x} \rVert < \epsilon $ for $0 \leq t \leq \infty$.
\end{definition}

\begin{definition} \label{def_stable_asym}
\textbf{(Asymptotic Stability)} \citep{glendinning1994stability} System (\ref{dynamic_system}) is \textit{asymptotic stable} if it is Lyapunov stable, and there exists a $\delta > 0$ such that whenever $\lVert x(0) - \Bar{x} \rVert \leq \delta$, we have $\lim_{t\to\infty} \lVert x(t) - \Bar{x} \rVert = 0$.
\end{definition}
\vspace{-0.05in}
Note that a dynamical system can be Lyapnuov stable but not asymptotic stable. However, every asymptotic stable dynamical system is Lyapnuov stable.


The field of control theory has studied how to drive dynamical systems to desired states. This can be achieved through the addition of a `controller' to allow influence over the dynamical system's evolution, for example creating an equilibrium at some desired state, and making the dynamical system stable around it.
% and encouraging convergence to that equilibrium.

\begin{definition} \textbf{(Controller)} \citep{brogan1991modern}
    A \textit{controller} of a dynamical system is a function $u(t)$ such that
    \begin{equation}
        \frac{d x(t)}{dt} = f(x(t)) +u(t) \label{dynamic_control} .
    \end{equation}
\end{definition}
The equilibrium and stability criteria introduced for dynamical system (\ref{dynamic_system}), equally apply to this controlled dynamical system (\ref{dynamic_control}). In order to analyze the stability of a controller $u(t)$ of the controlled dynamical system given an equilibrium $\Bar{x}$, the following result will be useful.
% \tp{make sure stability properties also links to system 2.}
% To evaluate controller $u(t)$ in terms of stability, the following theorem establishes stability analysis with regard to dynamical system (\ref{dynamic_control}) on equilibrium $\Bar{x}$.

% To evaluate controller $u(t)$ in terms of stability, the following theorem establishes stability analysis with regard to dynamical system (\ref{dynamic_control}) on equilibrium $\Bar{x}$.


\begin{theorem} \label{stabletheorem}\textbf{(Principle of Linearized Stability)} \citep{la1976stability}
    A controlled dynamical system (\ref{dynamic_control}) with equilibrium $\Bar{x}$ is asymptotically stable if all eigenvalues of $\mathbb{J}(f(\Bar{x}) + u(t))$ have negative real parts, where $\mathbb{J} (f(\Bar{x}) + u(t))$ represents the Jacobian of $f(x(t)) + u(t)$ evaluated at $\Bar{x}$.
    % Given a dynamical system (\ref{dynamic_control}) with equilibrium $\Bar{x}$, this system is asymptotically stable if all eigenvalues of $\mathbb{J}(f(\Bar{x}) + u(t))$ have negative real parts, where $\mathbb{J} (f(\Bar{x}) + u(t))$ represents the Jacobian of $f(x(t)) + u(t)$ evaluated at $\Bar{x}$.
\end{theorem} 
% \junz{lineared stability is not explained.}

\begin{corollary} \label{coro}
    If $\mathbb{J}(f(\Bar{x}) +u(t))$ has positive determinant and negative trace, all its eigenvalues have negative real parts and the system is asymptotically stable. %Theorem \ref{stabletheorem} also holds.
   
    % If $\mathbb{J}(f(\Bar{x}) +u(t))$ has positive determinant and negative trace, all eigenvalue of $\mathbb{J}(f(\Bar{x}) + u(t))$ have negative real parts, therefore theorem \ref{stabletheorem} also holds.
\end{corollary}

==> Styles/input/3-GAIL2dynamic.tex <==
\section{Analyzing GAIL as a Dynamical System} \label{sec:dynamic}
In this section, we study the training stability of GAIL through the lens of control theory. We derive the differential equations governing the training process of GAIL, framing it as a dynamical system. Then, we analyze the convergence of GAIL and find that it cannot converge to desired equilibrium due to the entropy term. For simplicity, we limit the theoretical analysis to the original GAIL\citep{ho2016generative} among many variants \citep{fu2017learning, jena2021augmenting, xiao2019wasserstein, kostrikov2018discriminator, swamy2022minimax}, while the controller proposed in the next section is general.
%The theoretical analysis in this section proves the training process of GAIL is unstable under general setting, which motivates our designed controller in Sec. \ref{control} that pushes GAIL to desired equilibrium.

\subsection{GAIL Dynamics}
% Given an action space $\mathcal{A}$ and a state space $\mathcal{S}$, 
GAIL consists of a learned generative policy $\pi_\theta : \mathcal{S} \rightarrow \mathcal{A}$ and a discriminator $D_\omega : \mathcal{S} \times \mathcal{A} \rightarrow (0,1)$. The discriminator estimates the probability that an input state-action pair is from the expert policy, rather than the learned policy.
% Consisting of a generative policy $\pi_\theta : S \rightarrow A$ and a discriminator $D_\omega : S \times A \rightarrow (0,1)$ \tp{do we want these () or []?}, 
GAIL alternatively updates the policy and discriminator parameters, $\theta$ and $\omega$. (The parameter subscripts are subsequently dropped for clarity.)
The GAIL objective \citep{ho2016generative} is $
\mathbb{E}_\pi[\log (D(s, a))]+\mathbb{E}_{\pi_E}[\log (1-D(s, a))]-\lambda H(\pi)$, where $\pi_E$ is the expert demonstrator policy, $\pi$ is the learned policy, and $H(\pi) \equiv \mathbb{E}_\pi [-\log \pi(a|s)]$ is its entropy. Respectively, the objective functions for the discriminator and policy (to be maximized and minimized respectively) are,
% \tp{removed entropy H, we never refer to it again}
% where $D$ is the discriminator that takes a state-action pair and outputs the probability of this state-action pair from the expert policy. $\pi$ is the policy representing the generator, $\pi_E$ is the given expert policy, and $H(\pi) \equiv \mathbb{E}_\pi [-\log \pi(a|s)]$ is the casual entropy of policy $\pi$. Respectively, the objective functions for the discriminator and generator can be written as
\begin{equation}
\begin{aligned} \label{obj1}
% \max_D V_D(D,\pi) &= \mathbb{E}_\pi [\log D(s,a)] + \mathbb{E}_{\pi_E}[\log(1-D(s,a))] \\
% \min_\pi V_\pi(D,\pi) &= \mathbb{E}_\pi[\log D(s,a)] - \lambda \mathbb{E}_\pi[-\log\pi (a\vert s)].
 V_D(D,\pi) &=  \mathbb{E}_\pi [\log D(s,a)] + \mathbb{E}_{\pi_E}[\log(1-D(s,a))] \\
 V_\pi(D,\pi) &=  \mathbb{E}_\pi[\log D(s,a)] - \lambda \mathbb{E}_\pi[-\log\pi (a\vert s)].
\end{aligned}
\end{equation}
% \tp{removing $V_1 V_2$ notation everywhere $\to V_D V_\pi$}
%\tp{I don't follow why $\frac{d D(t)}{d t}=\frac{\partial V_D(D, \pi)}{\partial D}$. What does $\frac{d D(t)}{d t}$ even mean? How the output of the discriminator for a given s, a changes over training? Also I think we should write $\partial D(t)$}
%\tj{$frac{d D(t)}{d t}$ refers to how the discriminator function changes with respect to time. Since we are using gradient step update, this is equivalent to how the objective functions is changed with respect to D. Here in Eq 5 we treat D as a function itself, but later on in Eq 12 we treat D(t) as a real-valued function for given state action pair in simplified setting for stability analysis. Similar for $\pi$。}
To describe GAIL as a dynamical system, we express how $\pi$ and $D$ evolve during training. For the analysis to be tractable, we study the training dynamics from a variational perspective, by directly considering the optimization of $\pi$ and $D$ in their respective \textit{function spaces}. This approach has been used in other theoretical deep learning works~\cite{ja2018,goodfellow2014generative,mescheder2018training} to avoid complications of the parameter space. 
% This assumption is somewhat crude but can nevertheless yield some useful insights. 
% \jianfei{better way to say this?}

We start by considering optimizing Eq.~(\ref{obj1}) with functional gradient descent with discrete iterations indexed by $m$: 
% \vspace{-0.1in}
    $D_{m+1}(s, a)=  D_{m}(s, a) + \beta  \frac{\partial V_D(D_m, \pi_m)}{\partial D_m(s, a)}$, and $ \pi_{m+1}(a|s)=  \pi_{m}(a|s) - \beta  \frac{\partial V_\pi(D_m, \pi_m)}{\partial \pi_m(a|s)}$,
% \vspace{-0.05in}
 where $\beta$ is the learning rate, $m$ the discrete iteration number, $\frac{\partial V_D(D_m, \pi_m)}{\partial D_m(s, a)}$ (similarly for $\frac{\partial V_\pi(D_m, \pi_m)}{\partial \pi_m(a|s)} $) is the \textit{functional derivative} \citep{lafontaine2015introduction} defined via $\partial V_D(D_m, \pi_m) = \int  \frac{\partial V_D(D_m, \pi_m)}{\partial D_m(s, a)} \partial D_m (s, a) \; ds \; da$, which implies the total change in $V_D$ upon variation of function $D_m$ is a linear superposition \citep{greiner2013field} of the local changes summed over the whole range of $(s,a)$ value pairs.
%The objective in Eq.~(\ref{obj1}) can be optimized in function space using gradient based method,
% \begin{equation} \label{gd}
%     \begin{aligned}
% D_{m+1}(s, a)&=  D_{m}(s, a) + \beta \times \frac{\partial V_D(D_m, \pi_m)}{\partial D_m(s, a)},
% \pi_{m+1}(a|s)&=  \pi_{m}(a|s) - \beta \times \frac{\partial V_\pi(D_m, \pi_m)}{\partial \pi_m(a|s)},
%In our theoretical analysis, we directly consider the updates of $\pi$ and $D$ in their respective \textit{function spaces}. 
% We leverage the variational method to compute the differential equation from the objective function of the generator and discriminator to get the training dynamic of GAIL. 
%In a variational perspective, 
% Denote $\frac{\partial V_D(D, \pi)}{\partial D}$ to be the gradient of $V_D(D, \pi)$ with respect to the discriminator $D$, and $\frac{\partial V_\pi(D,\pi)}{\partial \pi}$ to the gradient of $ V_\pi(D,\pi)$ with respect to the policy generator $\pi$.
% \left.\frac{\partial V_\pi(D_m, \pi_m)}{\partial \pi_m}\right|_{s,a},
% \end{aligned}
% \end{equation}

% \tj{\begin{equation} 
%     \begin{aligned}
% D_{m+1}(s, a)&\leftarrow D_{m}(s, a) + \beta \times \frac{\partial V_D(D_m(s,a), \pi_m)}{\partial D_m}, \nonumber\\
% \pi_{m+1}(a|s)&\leftarrow \pi_{m}(a|s) - \beta \times \frac{\partial V_\pi(D_m, \pi_m(a|s))}{\partial \pi_m} \nonumber
% \end{aligned}
% \end{equation}
% }

% Consider the continuous-time limit (a.k.a., gradient flow) of Eq. (\ref{gd}). 
% As $\beta \rightarrow 0$, we can replace the iteration number $m$ with the continuous time $t:=\beta m$, such that
% In the continuous-time limit (`gradient flow'), Eq. (\ref{gd}) can be represented by the functional derivative,  


We then consider the limit $\beta\rightarrow 0$, where discrete dynamics become continuous (`gradient flow') $
\frac{d D_{t}(s, a)} {dt} = \frac{\partial V_D(D_t, \pi_t)}{\partial D_t(s, a)} ,$ and $
\frac{d \pi_{t}(a|s)}{ dt} = \frac{-\partial V_\pi(D_t, \pi_t)}{\partial \pi_t( a|s)}$. 
%This is a dynamical system that portraits the gradient based update of the discriminator and the policy generator.
% where $\beta$ is the learning rate and $m$ the discrete iteration number. \tj{$\frac{\partial V_D(D_m, \pi_m)}{\partial D_m(s, a)}$ (similarly for $\frac{\partial V_\pi(D_m, \pi_m)}{\partial \pi_m(a|s)} $)  is the \textit{functional derivative} \citep{lafontaine2015introduction} defined such that $\partial V_D(D_m, \pi_m) = \int d s d a \frac{\partial V_D(D_m, \pi_m)}{\partial D_m(s, a)} \partial D_m (s, a)$, which implies the total change in $V_D$ upon variation of function $D_m$ is a linear superposition \citep{greiner2013field} of the local changes summed over the whole range of $(s,a)$ value pairs.}
% % Consider the continuous-time limit (a.k.a., gradient flow) of Eq. (\ref{gd}). 
% % As $\beta \rightarrow 0$, we can replace the iteration number $m$ with the continuous time $t:=\beta m$, such that
% In the continuous-time limit (`gradient flow'), Eq. (\ref{gd}) can be represented by the functional derivative,  \tj{In the continuous-time limit (`gradient flow'), we can portray the gradient based update of the discriminator and the policy generator as a dynamical system, }
% $
% \frac{d D_{t}(s, a)} {dt} = \frac{\partial V_D(D_t, \pi_t)}{\partial D_t(s, a)} ,
% \frac{d \pi_{t}(a|s)}{ dt} = \frac{-\partial V_\pi(D_t, \pi_t)}{\partial \pi_t( a|s)}.$
% \frac{\partial D_{t}}{\partial t} = \frac{\partial V_\pi(D_t, \pi_t)}{\partial D_t},\\
% \frac{\partial \pi_{t}}{\partial t} = \frac{\partial V_D(D_t, \pi_t)}{\partial \pi_t},
%Do a reparameterization $D_t:=D_{\alpha m}$ and let $\alpha\rightarrow 0$, we get...
Formally, we consider the evolution of the discriminator function $D_t: \mathcal S\times \mathcal A\rightarrow \mathbb R$ and the policy generator $\pi_t: \mathcal{S} \rightarrow \mathcal{A}$ over continuous time $t$ rather than discrete time $m$. We derive the training dynamic of GAIL in the following theorem. 
% Similarly to \citet{Luo2023Stable}, we can use the variational method to take the derivative of the above objective functions with respect to time $t$ to get the differential equations representing the training dynamic of the discriminator and the generator. 
% $D_t$: function
% $D_t(s, a)$: function evaluated at $(s, a)$
% Let $D(t) \triangleq D(s,a,t)$ and $\pi(t) \triangleq  \pi(a|s, t)$ to represent the discriminator and generator networks, respectively, at training time $t$. Denote $\frac{\partial V_D(D, \pi)}{\partial D}$ to be the gradient of $V_D(D, \pi)$ with respect to the discriminator $D$, and $\frac{\partial V_\pi(D,\pi)}{\partial \pi}$ to the gradient of $ V_\pi(D,\pi)$ with respect to the policy generator $\pi$.  
% where we have made explicit the dependence of the discriminator and generator functions on training time $t$, $D_t := D(s,a,t)$ and $\pi_t :=  \pi(a|s, t)$, but dropped their dependence on $s$ and $a$ to keep notation uncluttered. 
% The training dynamic of GAIL can be written as (detailed in appendix \ref{lemma2}) 

\begin{theorem}
    The training dynamic of GAIL takes the form (detailed proof in Appendix Lemma \ref{lemma2})
    \begin{gather} 
\frac{d D_t(s, a)}{d t}=\frac{\rho_{\pi_t}(s)\pi_t(a|s)}{D_t(s, a)}-\frac{\rho_{\pi_E}(s)\pi_E(a|s)}{1-D_t(s, a)},~~~~\\
\frac{d \pi_t(a | s)}{d t}=-\rho_{\pi_t}(s) A^{\pi_t}(s,a)\label{bianfen2}.
% \frac{\partial D_t}{\partial t}=\frac{\partial V_D(D_t, \pi_t)}{\partial D_t}=\frac{\rho_{\pi_t}(s)\pi_t(a|s)}{D_t}-\frac{\rho_{\pi_E}(s)\pi_E(a|s)}{1-D_t}\label{bianfen1}\\
% \frac{\partial \pi_t}{\partial t}=\frac{\partial V_\pi(D_t,\pi_t)}{\partial \pi_t}=\rho_{\pi_t}(s) A^{\pi_t}(s,a)\label{bianfen2},
\end{gather}
\end{theorem}

% We derive these functional derivatives in Appendix Lemma \ref{lemma2}, which take the form, 
% Similarly to \citet{Luo2023Stable}, we can use the variational method to take the derivative of the above objective functions with respect to time $t$ to get the differential equations representing the training dynamic of the discriminator and the generator. Let $D(t) \triangleq D(s,a,t)$ and $\pi(t) \triangleq  \pi(a|s, t)$ to represent the discriminator and generator networks, respectively, at training time $t$. Denote $\frac{\partial V_1(D, \pi)}{\partial D}$ to be the gradient of $V_1(D, \pi)$ with respect to the discriminator $D$, and $\frac{\partial V_2(D,\pi)}{\partial \pi}$ to the gradient of $ V_2(D,\pi)$ with respect to the policy generator $\pi$.  We introduce time $t$ into this notation because both the generator and discriminator network vary with respect to the time $t$. Since $\pi_E$ is constant through the training dynamic, we intentionally omit the symbol $t$ for expert policy. The training dynamic of GAIL can be written as (detailed in appendix \ref{lemma2})
% \jianfei{here, the notation of $\pi$ in equation and definition still do not match. you have 3 notations: $\pi_t$, $\pi((a|s), t)$, and $\pi_t(a|s)$. Moreover, what is $\rho_{\pi_t}(s)$? where is $a$?¬
% }
% \begin{gather} 
% \frac{d D_t(s, a)}{d t}=\frac{\rho_{\pi_t}(s)\pi_t(a|s)}{D_t(s, a)}-\frac{\rho_{\pi_E}(s)\pi_E(a|s)}{1-D_t(s, a)},~~~~
% \frac{d \pi_t(a | s)}{d t}=-\rho_{\pi_t}(s) A^{\pi_t}(s,a)\label{bianfen2},
% % \frac{\partial D_t}{\partial t}=\frac{\partial V_D(D_t, \pi_t)}{\partial D_t}=\frac{\rho_{\pi_t}(s)\pi_t(a|s)}{D_t}-\frac{\rho_{\pi_E}(s)\pi_E(a|s)}{1-D_t}\label{bianfen1}\\
% % \frac{\partial \pi_t}{\partial t}=\frac{\partial V_\pi(D_t,\pi_t)}{\partial \pi_t}=\rho_{\pi_t}(s) A^{\pi_t}(s,a)\label{bianfen2},
% \end{gather}
% where $\rho_{\pi_t}(s)$ and $\rho_{\pi_t}(s)\pi_t(a|s)$ are respectivelt the state-action occupancy
% where $D_t$ and $\pi_t$ to be the discriminator and policy functions at time $t$, 
% Here $\rho_{\pi_t}$ and $A^{\pi_t}$ are the state occupancy and the advantage function of the policy $\pi_t$ (Section \ref{setting}). 
% Since the demonstrator policy $\pi_E$ is constant through the training dynamic, we omit its dependence on $t$. 
 % \jianfei{make this a theorem?}

% We slightly abuse notation with $\rho_{\pi_t}(s)$ meaning the state-only occupancy $\rho_{\pi_t}(s) \sum_{n=0}^{\infty} \gamma^n P (s_n = s | \pi_t)$.\jianfei{still needs polishing}
% where $\rho_{\pi_t}(s)\pi_t(a|s)$ is the occupancy measure of policy $\pi_t$, and $A^{\pi_t}$ is the advantage function, defined in Section \ref{setting}.
% , such that
% \begin{gather*}
% \rho_{\pi_t}(s) :=  \sum_{n=0}^{\infty} \gamma^n P(s_n=s|\pi_t) \\ 
% \rho_{\pi_t}(s)\pi_t(a|s) := \pi_t(a|s)\rho_{\pi_t}(s) \\
% \mathbb{E}_\pi[g(s,a)] = \int_s \int_a \rho_\pi(s,a) g(s,a) dads\\
% Q^{\pi(t)}(s, a) := \mathbb{E}_{\pi(t)}[c(\bar{s},\bar{a}) + \lambda \log \pi(t)(\bar{a}|\bar{s})| s_0 = s, a_0 = a] \\  A^{\pi(t)}(s,a):= Q^{\pi(t)}(s,a) - \mathbb{E}_{\pi(t)}[Q^{\pi(t)}(s,a)]. \label{eq:advantage}
% \end{gather*} 

% \huayu{
% \begin{gather} 
% \frac{d D(s,a,t)}{d t}=\frac{\partial V_1(D, \pi)}{\partial D}=\frac{\rho_{\pi_t}(s)\pi_t(a|s)}{D(s,a,t)}-\frac{\rho_{\pi_E}(s)\pi_E(a|s)}{1-D(s,a,t)}\label{bianfen1}\\
% \end{gather}
% where
% \begin{gather} 
% \rho_{\pi_t}(s)\pi_t(a|s) := \pi(a|s,t) \rho_{\pi_t}(s) := \pi(a|s,t) \sum_{n=0}^{\inf} \gamma^n P(s_n=s|\pi_t)
% \end{gather}
% 0. I'm basically certain I'm correct for this quation.
% 1. please note that in RL there is also an episode timestep termed t. I switch that to n here.
% 2. For a detailed explanation of $\rho$, refer to GAIL paper, page 3
% }
% \tj{Following the notation from \cite{lafontaine2015introduction}, we denote $\nabla V_D(D, \pi) &= (\nabla_{D} V_D, \nabla_{\pi} V_D)(D, \pi)$ and $\nabla V_{\pi}(D, \pi) &= (\nabla_{D} V_{\pi}, \nabla_{\pi} V_{\pi})(D, \pi)$ as the functional gradient for $V_D$ and $V_\pi$ with respect to $D$ and $\pi$. Then the following holds for all $(s,a)$ pairs. \begin{equation}
%     \begin{aligned}
%         % \text{Denote}\ \nabla V_D(D, \pi) &= (\nabla_{D} V_D, \nabla_{\pi} V_D)(D, \pi)  \\
%         % \text{Denote}\ \nabla V_{\pi}(D, \pi) &= (\nabla_{D} V_{\pi}, \nabla_{\pi} V_{\pi})(D, \pi)  \\
%         D_{m+1} &=D_{m} + \beta \times \left.\nabla_{D} V_D\right|_{D_m, \pi_m}, \nonumber\\
%         \pi_{m+1} &= \pi_{m} - \beta \times \left.\nabla_{\pi} V_\pi\right|_{D_m, \pi_m}, \nonumber \\
%         \frac{d D_{t}}{  dt}   &= \left.\nabla_{D} V_D\right|_{D_t, \pi_t}\\
%        \frac{ d \pi_{t}} {dt} &= -\left.\nabla_{\pi} V_\pi\right|_{D_t, \pi_t}.\\
%         \frac{d D_t}{d t} &=\left.\nabla_{D} V_D\right|_{D_t, \pi_t}=\frac{\rho_{\pi_t}}{D_t}-\frac{\rho_{\pi_E}}{1-D_t}\\
%         \frac{d \pi_t}{d t} &=- \left.\nabla_{\pi} V_\pi\right|_{D_t, \pi_t}=-\rho_{\pi_t} A^{\pi_t},
%     \end{aligned}
% \end{equation}}


% \huayu{
% \begin{gather} 
% \frac{d \pi((a|s),t)}{d t}=\frac{\partial V_2(D,\pi)}{\partial \pi}=\rho_{\pi_t}(s) \log D(s,a,t)+\lambda\rho_{\pi_t}(s)\log\pi(a|s,t)+\lambda\rho_{\pi_t}(s)\label{bianfen2},
% \end{gather}
% 0. This is correct only if we assume that $\pi$ does not influence $\rho_\pi(s)$ ($\frac{d \rho_\pi(s)}{d \pi} = 0$), which is acceptable in RL, because many papers do this. But I'm not sure if this is acceptable in this paper.}

% \huayu{
% \begin{gather} 
% \frac{d \pi((a|s),t)}{d t}=\frac{\partial V_2(D,\pi)}{\partial \pi}=\rho_{\pi_t}(s) Q(s,a,t)\label{bianfen2},
% \end{gather}
% where
% \begin{gather} 
% Q(s,a,t):= E_\pi[\log D(s,a,t) + \lambda \log \pi(a|s,t)],
% \end{gather}
% 0. This is a guessed solution if we formally consider ($\frac{d \rho_\pi(s)}{d \pi} \neq 0$). However, I'm not sure if this is the correct solution.}


% For simplicity, we define $x(t) = D(s,a,t)$ , $y(t) = \pi(a|s, t)$ and $E = \pi_E(a|s)$. We then have the following dynamic equations:
% \begin{gather} 
% \frac{d x(t)}{d t}=\frac{y(t)}{x(t)}+\frac{E}{x-1}\label{dyx}\\
% \frac{d y(t)}{d t}=\frac{y(t)}{x(t)}+\lambda \log y(t)+\lambda \label{dyy}.
% \end{gather}

% Since the ideal goal of GAIL is to estimate expert policy $\pi_E$ with our policy generator, and let discriminator unable to distinguish between expert policy and generated policy, which is $\pi^*(a|s, t) = \pi_E(a|s)$ and $D^*(s, a, t) = \frac{1}{2}$ as t goes to infinity. Ideally we expect 
% \begin{gather} 
%     \lim_{t \to \infty} x(t) = \frac{1}{2}  \label{eqx} \\
%      \lim_{t \to \infty} y(t) = \pi_E(a|s) \label{eqy}
% \end{gather}
% \jianfei{the notations are somewhat unconventional. $x(t)$ is a function $\mathcal S\times \mathcal A\rightarrow \R$, $\frac{1}{2}$ is a real number. It is strange that $x(t)=\frac{1}{2}$. Find proper notations from functional analysis textbooks?}


% \subsection{GAIL Does not Converge} 
\subsection{On the Convergence of GAIL} \label{sec:notconverge}
% \tj{TODO: change the title and wording to make it less strong}

% Throughout the training process of GAIL, we expect our policy generator to estimate expert policy, and our discriminator becomes indistinguishable between the expert and generated policy. In this manner, We define the \textit{goal functions} for the discriminator and the policy generator to be
Now, we study the optimization stability of GAIL using the dynamical system Eq.~(\ref{bianfen2}). 
The desirable outcome of the GAIL training process, is for the learned policy to perfectly match the expert policy, and the discriminator to be unable to distinguish between the expert and learned policy. 
% This \textit{desired state} is defined as,
% \begin{gather} \label{fix}
%     D^*_t(s, a)= \frac{1}{2} ,\\
%     \pi^*_t(a|s) = \pi_E.
% \end{gather}
% \tp{might be worth formatting this as a formal defn given how much we later refer to it?}
\begin{definition} \label{def_desired_state} \textbf{(Desired state)} 
    We define the desired outcome of the GAIL training process as the discriminator and policy reaching 
    $
    D^*_t(s, a)= \frac{1}{2} , \pi^*_t(a|s) = \pi_E(a|s). \nonumber $
\end{definition}
% \tp{check, does D(s,a)=1/2 hold for any s, a, or does it have to be from support of expert or something?}

We are interested in understanding whether GAIL converges to the desired state. As discussed in Sec.~\ref{sec:dynamical-systems},  the desired state should be the equilibrium of the dynamical system Eq. (\ref{bianfen2}) for such convergence. According to Def. \ref{eqdef}, the dynamical system should equal to zero at this point, but we present the following theorem (proved in Proposition \ref{propneq0} and \ref{propneq1}):
% If this desired state is an equilibrium, 
% Substituting these desired states into the dynamical system described by Eq. (\ref{bianfen1}) \& (\ref{bianfen2}) and get 
% We substitute these desired states, Eq. (\ref{fix}) \& (\ref{noteq0}), for the discriminator and the policy generator to the dynamical system (Eq. (\ref{bianfen1}) and Eq. (\ref{bianfen2})) and get (detailed in appendix \ref{propneq0} and \ref{propneq1})
% \jianfei{make this a theorem?}
\begin{theorem}  
    The training dynamics of GAIL does not converge to the desired state, and we have 
    \begin{equation}\label{noteq0}
    \frac{d D^*_t(s,a)}{d t} = \frac{\rho_{\pi^*_t}(s)\pi^*_t(a|s)}{D^*_t}-\frac{\rho_{\pi_E}(s)\pi_E(a|s)}{1-D^*_t}=0,   \frac{d \pi^*_t(a|s)}{d t} = -\rho_{\pi^*_E}(s) A^{\pi^*_E}(s,a) \neq 0.
\end{equation}
\end{theorem}
% \begin{gather}
% \frac{d D^*_t(s,a)}{d t} = \frac{\rho_{\pi^*_t}(s)\pi^*_t(a|s)}{D^*_t}-\frac{\rho_{\pi_E}(s)\pi_E(a|s)}{1-D^*_t}=0, \label{eq0}
% \frac{d \pi^*_t(a|s)}{d t} = -\rho_{\pi^*_E}(s) A^{\pi^*_E}(s,a) \neq 0. \label{noteq0}
% \end{gather}
% \tp{should 2nd eq be -ve?}
\vspace{-0.15in}
Hence, the desired state is not an equilibrium, and GAIL will not converge to it.
Since $\frac{d \pi^*_t(a|s)}{d t}\neq 0$, even if the system is forced to the desired state, it will drift away from it.
% Inspecting Proposition \ref{propneq0}, 
We find that the non-equilibrium result is due to the entropy term $\lambda H(\pi)$, and an equilibrium could be achieved by simply setting $\lambda=0$ (Corollary \ref{corr_no_entropy}). However, the  entropy term is essential since it resolves the exploration issue and prevents over-fitting.
Therefore, we aim to design a controller that not only keeps the entropy term but also improves the theoretical convergence guarantee.



% \tp{ideally would have another proof to show that without entropy term it does equal zero}
% \tj{I mentioned the entropy term at the beginning of this section. Maybe we need to talk about it again here.}
% Therefore, as suggested in remark \ref{convergeremark}, GAIL is unable to converge to the goal functions, which means the policy generator cannot converge to the expert policy.
% Since Eq. (\ref{noteq0}) does not equal 0, according to def. \ref{eqdef}, our goal functions are not equilibrium points for GAIL's training dynamic. Therefore, as suggested in remark \ref{convergeremark}, GAIL is unable to converge to the goal functions, which means the policy generator cannot converge to the expert policy.
% \tp{maybe add a proof sketch? It is straightforward to see that Eq. \ref{eq0} holds when $\pi_* = \pi_E$ and $D^*=1/2$. In Eq. \ref{noteq0}, there must exist $s$ where $\rho_{\pi^*_t}(s)>0$, in which case $A^{\pi^*_t}(s,a)$ should equal zero. However, reviewing Eq. \ref{eq:advantage}, the ... I'm confused again. Maybe the argument is more complex than I thought. What if the expert policy is fully deterministic, so entropy is always zero. does the expert policy w a little entropy added lead to a equilibrium? }

==> Styles/input/4-control.tex <==
% \section{Convergence and Stability of GAIL} \label{control}
\section{Controlled GAIL} \label{control}


Having shown in Section \ref{sec:dynamic} that GAIL does not converge to the desired state, this section considers adding a controller to enable the convergence. 
%We propose a simple ``one-step GAIL'' setting to simply the analysis. 
We design controllers for both the discriminator and the policy. We show that this controlled system converges to the desired equilibrium and also achieves asymptotic stability in a simplified ``one-step'' setting. 
%We then propose a pragmatic variant of this controller to be used in practise which we name C-GAIL.\jianfei{TODO}



% In this section, we start with the dynamical system of GAIL derived in Section \ref{sec:dynamic} and prove that GAIL is unable to converge the policy generator to the expert policy. We then further analyze the training dynamic for one step of update for a state-action pair and propose controllers for both the discriminator and the policy generator. Our controllers can not only successfully converge to the desired equilibrium but also achieve asymptotic stability.



\subsection{Controlling the Training Process of GAIL} \label{sec:controlller}
Establishing the convergence for GAIL is challenging since the occupancy measure $\rho_\pi$ involves an expectation over the states generated by playing the policy $\pi$ for infinite many steps. We simplify the analysis by truncating the trajectory length to one: we only consider the evolution from timestep $n$ to $n+1$. We refer this simplified setting as ``one-step GAIL'', and the convergence guarantee of our proposed algorithm will be established in this simplified setting. 
%To design a controller for GAIL, we consider a single environment timestep $n$ of the trajectory with state $s_n$ and action $a_n$ -- we refer to this as the `one-step GAIL'. 
Let $p(s)$ be the probability of the state at $s$ on timestep $n$. The objectives for the discriminator and the policy can then be simplified as, 
% To further analyze the stability of GAIL, we zoom in on our objective function for policy within one step. Considering step $n$ of the trajectory with state $s_n$ and taking action $a_n$, and letting $p(s)$ be the probability of the state 
% at $s$ on time step $k$, then the objective functions for the discriminator and the policy generator at step $n$ can be written as 
\begin{align*}
\tilde{V}_{D}(D, \pi)&= \int_{a}\int_{s} p(s) \pi(a|s)\log D(s,a) + \pi_E(a|s)\log(1-D(s,a))\;ds \;da , \\
\tilde{V}_{\pi}(D, \pi) &= \int_{a}\int_{s} p(s) \pi(a|s)\log D(s,a) + \lambda p(s) \pi(a|s) \log\pi(a|s)\;ds \;da .
\end{align*}

% \begin{equation}
% \begin{split}
% \begin{aligned}
% \tilde{V}_{D}(D, \pi) = \int_{a_n}\int_{s_n} p(s_n) \pi(a_n|s_n)\log D(s_n,a_n)dsda \\ + \int_{a_n}\int_{s_n} p(s_n) \pi_E(a_n|s_n)\log(1-D(s_n,a_n))dsda , \\  \nonumber
% \tilde{V}_{\pi}(D, \pi) = \int_{a_n}\int_{s_n} p(s_n) \pi(a_n|s_n)\log D(s_n,a_n)dsda \\ + \lambda\int_{a_n}\int_{s_n} p(s_n) \pi(a_n|s_n) \log(\pi(a_n|s_n))dsda . \nonumber
%    \end{aligned}
%     \end{split}
% \end{equation}
% One interpretation of this is as an MDP with $\gamma=0$. 
% Eq. (\ref{bianfen1}) \& (\ref{bianfen2}) can then be rewritten (replacing $V_{D}(D, \pi), V_{\pi}(D, \pi)$ with $\tilde{V}_{D}(D, \pi), \tilde{V}_{\pi}(D, \pi)$),
The gradient flow dynamical system of these functions is,
% We compute the one-step training dynamic for policy generator by taking derivative with respect to function $D$ and policy generator $\pi$ to get 
\begin{align}
\frac{d D_t(s, a)}{dt} 
&= \frac{p(s) \pi_t(a|s)}{D_t(s, a)} + \frac{p(s) \pi_E(a|s)}{D_t(s, a) -1}, \label{simD}\\
 \frac{d\pi_t(a|s)}{dt}     
    &= -p(s) (\log D_t(s, a) +  \lambda \log\pi_t(a|s) + \lambda). \label{simG}
    % \vspace{-0.05in}
\end{align}

% \begin{equation} \label{simD}
% \begin{split}
% \begin{aligned}
% \frac{d D_t(s, a)}{dt} 
% = \frac{p(s) \pi_t(a|s)}{D_t(s, a)} + \frac{p(s) \pi_E(a|s)}{D_t(s, a) -1}, 
% \end{aligned}
%     \end{split}
% \end{equation}
% \begin{equation} \label{simG}
% \begin{split}
% \begin{aligned}
%     \frac{d\pi_t(a|s)}{dt}     
%     = -p(s) (\log D_t(s, a) +  \lambda \log\pi_t(a|s) + \lambda). 
%     \end{aligned}
%     \end{split}
% \end{equation}


% \huayu{The bracket here (eq.) seems strange to me.}
% \tj{For given $(s,a)$ pair, we have 
% \begin{equation} 
% \begin{split}
% \begin{aligned}
% \left.\frac{d D_t}{dt}\right|_{s, a}
% %= \frac{\partial V_{D}(D_t, \pi_t)}{\partial D_t(s, a)} 
% = \frac{p(s) \pi_t(a|s)}{D_t(s, a)} + \frac{p(s) \pi_E(a|s)}{D_t(s, a) -1}, 
% \end{aligned}
%     \end{split}
% \end{equation}
% \begin{equation} \label{simG}
% \begin{split}
% \begin{aligned}
%     \left.\frac{d\pi_t}{dt}\right|_{(s, a)} 
%     %= \frac{\partial V_{\pi}(D_t, \pi_t)}{\partial \pi}
%     = -p(s) (\log(D_t(s, a) +  \log(\pi_t(a|s) + 1). 
%     \end{aligned}
%     \end{split}
% \end{equation}
% }

% where $p(s)$ is the probability of state $s$ at step $n$.
With this ``one-step'' simplification, the GAIL dynamics now reveal a clearer structure. For a given $(s, a)$ pair, the change of $D(s, a)$ and $\pi(a | s)$ only depends on $D(s, a), \pi(a | s), p(s)$ and $\pi_E(a|s)$ for the same $(s, a)$ pair, without the need to access function values of other $(s, a)$ pairs. 
Therefore, we can decompose Eq.~(\ref{simD}) \& (\ref{simG}), which are ODEs of \emph{functions}, into a series of ODEs of \emph{scalar values}.
Each ODE only models the dynamics of two scalar values $(D(s, a), \pi(a | s))$ for a particular $(s, a)$ pair. 
We will add controller to the scalar ODEs, to asymptotically stabilize their dynamical system. 
% Once we prove that each scalar ODE is stable, we can extend/anticipate \jianfei{?} that the function ODE is stable.
Proving that each scalar ODE is stable suggests that the functional ODE will also be stable.
%\jianfei{like I said earlier, this actually needs a theorem to prove that $\forall (s, a)$, scalar ODEs are stable $\Rightarrow $ function ODE is stable. This might be tricky since we don't even have the definition for the stability of the function ODE} 
Note that such decomposition is not possible without the ``one-step'' simplification, since the evolution of $D$ and $\pi$ for all $(s, a)$ pairs is coupled through $\rho_\pi(s)$ and $A^\pi(s, a)$ in Eq.~(\ref{bianfen2}). 

% \tp{I'm struggling to follow the explanation/implications of the one step setting, but will trust others }
% the dynamics of $D(s, a)$ and $\pi(a | s)$ for each $(s, a)$ pair are independent. , and conclude that for each given $(s,a)$ pair, our controller is able to asymptotically stabilize its dynamical system.


% each for a particular $(s, a)$ pair, and analyze the stability of this system of ODEs of  for each pair individually

% Notice that though Eq.~(\ref{simD}) \& (\ref{simG}) are ODEs of functions $D$ and  $\pi$ respectively, 


% If the the system of ODEs for each $(s, a)$ is stable, the joint ODEs for the discriminator function $D$ and the policy distribution $\pi$ will also be stable. \tp{I'm fuzzy on why this holds -- is this obvious or is there something to cite to verify?} \tj{This does not necessarily hold. This is a gap we have from theory to pratice. However, in discrete state and action space I think it should hold.}
% Notice that though Eq.~(\ref{simD}) and Eq.~(\ref{simG}) are ODEs of functions $D$ and  $\pi$ respectively, the dynamics of $D(s, a)$ and $\pi(a | s)$ for each $(s, a)$ pair are independent. Therefore, we can decompose Eq.~(\ref{simD}) and Eq.~(\ref{simG}) to series of ODEs, each for a particular $(s, a)$ pair, and analyze the stability of this system of ODEs of $(D(s, a), \pi(a | s))$ for each $(s, a)$ pair separately. Hopefully, if the the system of ODEs for each $(s, a)$ is stable, the joint ODEs for the discriminator function $D$ and the policy distribution $\pi$ will also be stable.

Based on the above discussion, we now consider the stability of a system of ODEs for two scalar variables $(D(s, a), \pi(a | s))$. With $s, a$ given, we simplify the notation as $x(t) := D_t(s, a)$, $y(t) := \pi_t(s|a)$, $E:=\pi_E(a|s)$, $c := p(s)$, so each scalar ODE can be rewritten as,
% Next, we only need to consider the stability of a system of ODEs for two scalar variables $(D(s, a), \pi(a | s))$, rather than two functions. Without loss of generality, we consider the stability for a particular state $s$ and action $a$, and the analysis generalizes to all state-action pairs. Since $s, a$ are given, we simply the notation as $x(t) := D_t(s, a)$, $y(t) := \pi_t(s,a)$, $E:=\pi_E(a|s)$, $c := p(s)$, and rewrite our dynamical system as 
%Therefore, we define $x(t)$, $y(t)$ to be real-valued function evaluated at this state action pair, such that $x(t) = D(t)|_{(s, a)}$, $y(t) = \pi(t)|_{(s,a)}$, $E=\pi_E(a|s)$, $c = p(s)$, and rewrite our dynamical system as  
\begin{gather}
     \frac{dx (t)}{dt} = \frac{c y(t)}{x(t)} + \frac{c E}{x(t) - 1}, 
      \frac{dy (t)}{dt} = -c\log x(t) - c\lambda \log y(t) - c \lambda. \label{eq_yt_dt}
\end{gather}
% \tp{I'm confused why we needed the functional derivatives at all if we end up using these partial derivatives?}
% \tj{The partial derivative is only a intermediate step. Our concern is on the dynamical systems in forms of  Eq. 2}

We showed earlier that the GAIL dynamic in Eq. (\ref{bianfen2}) does not converge to the desired state. Similarly, neither does our simplified `one-step' dynamic in Eq. (\ref{eq_yt_dt}) converge to the desired state. We now consider the addition of controllers to push our dynamical system to the desired stated. Specifically, we consider linear negative feedback control \citep{boyd1991linear}, which can be applied to a dynamical system to reduce its oscillation. We specify our controlled GAIL system as,
% The training dynamic of GAIL in Eq. (\ref{bianfen1}) \& (\ref{bianfen2}) does not converge to the goal functions. Fortunately, in control theory, we can design controllers to push a dynamical system to given goal functions. For example, a linear negative feedback control \citep{boyd1991linear} can be applied to a dynamical system to reduce the oscillation of the system. We introduce our controlled system as
\begin{align}
\frac{\mathrm{d}x(t)}{\mathrm{d}t}&= \frac{c y(t)}{x(t)} + \frac{c E}{x(t) - 1}+u_1(t)\label{eqxu}\\
\frac{\mathrm{d}y(t)}{\mathrm{d}t}&=-c\log x(t) - c\lambda \log y(t) - c \lambda +u_2(t)\label{eqyu},
\end{align}
where $u_1(t)$ and $u_2(t)$ are the controllers to be designed for the discriminator and policy respectively. Since the derivative of the discriminator with respect to time evaluated at the desired state (Def. \ref{def_desired_state}) already equals zero, the discriminator is already able to reach its desired state. 
Nevertheless, the discriminator can still benefit from a controller to speed up the rate of convergence -- we choose a linear negative feedback controller for $u_1(t)$ to push the discriminator towards its desired state. 
% Therefore, we only need to design a linear negative feedback controller $u_1(t)$ for the discriminator to keep Eq. (\ref{eqxu}) equal to zero at the desired state. 
% \tp{why do we need anything for the discrim if it's already converging to what we needed?} \tj{To speed up the rate of convergence. Make sure to emphasize that.}
On the other hand, the derivative of the policy generator evaluated at its desired state in Eq. (\ref{eq_yt_dt}) does not equal zero. Therefore, $u_2(t)$ should be set to make Eq. (\ref{eqyu}) equal to zero evaluated at the desired state. We have designed it to cancel out all terms in Eq. (\ref{eq_yt_dt}) at this desired state, and also provide feasible hyperparameter values for an asymptotically stable system.
Hence, we select $u_1(t)$ and $u_2(t)$ to be the following functions,
% introduce an extra variable $\alpha$ to ensure the
% dynamical system as a whole is asymptotically stable. 
% Here we choose $u_1(t)$ and $u_2(t)$ to be the following functions,
% where $u_1(t)$ and $u_2(t)$ are the controllers for the discriminator and policy generator respectively. Since the derivative of the discriminator with respect to time evaluated at the goal function in Eq. (\ref{eq0}) already equals 0, the discriminator is possible to approach its goal function. Therefore, we only need to design a linear negative feedback controller $u_1(t)$ for the discriminator to keep Eq. (\ref{eqxu}) equal to 0 at the goal function. On the other hand, the derivative of the policy generator with respect to time evaluated at its goal function in Eq. (\ref{noteq0}) does not equal 0. Therefore, $u_2(t)$ should be able to adjust Eq. (\ref{eqyu}) to 0 evaluated at the goal function. Here we define $u_1(t)$ and $u_2(t)$ to be the following functions
\begin{gather}
    u_1(t) = -k(x(t)-\frac{1}{2}) \label{eq_u1}, \\
    u_2(t)= c\lambda \log E+c\log\frac{1}{2}+c\lambda + \alpha \frac{y(t)}{E} - \alpha,  \label{eq_u2}
\end{gather}
% \tp{should probably say where these functional forms come from -- are we just cancelling terms in 17 and 18 and then ensuring desired state sets it to zero? is this a standard ctrl theory thing to do?}
where $k, \alpha$ are hyper-parameters. Intuitively, as $k$ gets larger, the discriminator will be pushed harder towards the optimal value of $1/2$. This means the discriminator would converge at a faster speed but may also have a larger radius of oscillation. 
% To understand the convergence behavior of this controlled dynamical system, and provide bounds on the values of $k$ and $\alpha$, we will analyze its stability in the next section.

% where $k, \alpha$ are hyper-parameters introduced. Intuitively, as $k$ gets larger, the discriminator will get a higher punishment as it deviates from the optimal value, so the discriminator would converge at a faster speed but may also have a larger radius of oscillation. For a detailed convergence behavior analysis of controlled GAIL and specific bound on the range of $k$ and $\alpha$, we need to conduct stability analysis with respect to the controlled dynamical system.



\subsection{Analyzing the Stability of Controlled GAIL}
% \subsection{Asymptotically Stable of Controlled GAIL}
In this section, we apply Theorem \ref{stabletheorem} to formally prove that the controlled GAIL dynamical system described in Eq. (\ref{eqxu}) \& (\ref{eqyu}) is \textit{asymptotically stable} (Def. \ref{def_stable_asym}) and give bounds with $\lambda$, $\alpha$, and $k$.
% In this section, we formally prove that our controlled training dynamic of GAIL in Eq. (\ref{eqxu}) and Eq. (\ref{eqyu}) is \textit{asymptotically stable} and derive the bound of the relationship between $\lambda$ and $k$.

For simplicity, let us define $z(t) = (x(t), y(t))^\top$, and a function $f$ such that $f(z(t))$ is the vector
$\big[ \frac{c y(t)}{x(t)} + \frac{c E}{x(t) - 1}-k\left(x(t)-\frac{1}{2}\right) ,
    c\log \frac{1}{2} + c\lambda \log E  -c\lambda \log y(t) -c\log x(t) + \alpha \frac{y(t)}{E} - \alpha\big]^\top$.
% \begin{equation}
% \bigg[ \frac{c y(t)}{x(t)} + \frac{c E}{x(t) - 1}-k\left(x(t)-\frac{1}{2}\right) ,
%     c\log \frac{1}{2} + c\lambda \log E  -c\lambda \log y(t) -c\log x(t) + \alpha \frac{y(t)}{E} - \alpha\bigg]^\top
% \end{equation}
% \begin{equation}
% \begin{aligned}
% & \begin{pmatrix}
%     \frac{c y(t)}{x(t)} + \frac{c E}{x(t) - 1}-k\left(x(t)-\frac{1}{2}\right) \\
%     c\log \frac{1}{2} + c\lambda \log E  -c\lambda \log y(t) -c\log x(t) + \alpha \frac{y(t)}{E} - \alpha
%   \end{pmatrix}. \nonumber
% \end{aligned}
% \end{equation}
Therefore, our controlled training dynamic of GAIL in Eq. (\ref{eqxu}) and Eq. (\ref{eqyu}) can be transformed to the following vector form
\begin{equation} \label{vector}
    d (z(t)) =f(z(t))d t.
\end{equation}

% Given this set up, we prove in Appendix \ref{appB} that the following theorem holds.
    \begin{theorem} \label{thm_asym_stable}Let assumption \ref{assumption} hold. The training dynamic of GAIL in Eq. (\ref{vector}) is \textbf{asymptotically stable} (proof in  Appendix \ref{appB}).
    \end{theorem}


\begin{assumption} \label{assumption}
    We assume $\alpha, k \in \displaystyle \mathbb{R}, k>0$, $8c^2\lambda -8c\alpha -4c
        ^2 +ck\lambda -k\alpha > 0$, and  $\frac{k^2 +32c(-c\lambda + \alpha)}{32c} < 0$.
\end{assumption}

% \begin{assumption} \label{assumption}
%     We assume $\alpha, k \in \displaystyle \mathbb{R}, k>0$, 
%     % \tp{fixed R format. should alpha have to be $>0$?} \tj{Not Necessarily} 
%     and,
%     \begin{align} 
%     \text{(a)}& \;\;\;\;\;
%         8c^2\lambda -8c\alpha -4c
%         ^2 +ck\lambda -k\alpha > 0 \nonumber\\
%     \text{(b)}& \;\;\;\;\;       
%     \frac{k^2 +32c(-c\lambda + \alpha)}{32c} < 0 \nonumber
%     \end{align}
% \end{assumption}

% \tp{simplify (a) to $c\lambda  > \alpha$?} \\
% \tp{I think (a) is redundant actually. (c) simplifies to $c \lambda  - \frac{k^2}{32c} > \alpha$. Since $\frac{k^2}{32c}$ must be positive, (a) is a looser version of (c).}
% \tp{where do these come from? these bounds are a requirement to make the theorem work or has tj derived them or?}
% \tp{interesting that c crops up (state prob). is there some insight about how to set k and lambda based on the state space size or something? just thinking aloud}
% \tj{Let me show you how I derived it in discussion}
\textbf{Proof sketch.}
The first step in proving asymptotic stability of the system in Eq. (\ref{vector}), is to verify whether our desired state is an equilibrium (Def. \ref{eqdef}).
% To analyze the convergence and stability behavior of system Eq. (\ref{vector}), first we need to verify Def. \ref{eqdef} to make sure our desired state is an equilibrium.
We substitute the desired state, $z^*(t) = (\frac{1}{2}, E)^\top$, into system (\ref{vector}) and verify that $d (z^*(t)) = f(z^*(t)) = 0.$
% Notice that $z^*(t) = (\frac{1}{2}, E)\top$, then we substitute this goal function to system (\ref{vector}) and verify,
We then find the linearized system about the desired state $ d (z(t)) = \mathbb{J}(f(z^*(t))) z(t) d t.$ Under Assumption \ref{assumption}, we show that $det(\mathbb{J} (f(z^*(t)))) > 0$ and $trace(\mathbb{J} (f(z^*(t)))) < 0$. Finally we invoke Theorem \ref{stabletheorem} and Corollary \ref{coro} to conclude that the system in Eq. (\ref{vector}) is asymptotically stable. 
% We verify that when assumption \ref{assumption} are made, the $det(\mathbb{J} f(z^*(t))) > 0$ and $trace(\mathbb{J} f(z^*(t))) < 0$. Therefore we apply theorem \ref{stabletheorem} to prove Eq. (\ref{vector}) is asymptotically stable. 

% \begin{theorem}
%     (Proof in Appendix \ref{appB}) Let assumption \ref{assumption} hold. The training dynamic of GAIL in Eq. (\ref{vector}) is \textbf{asymptotically stable}.
%  \end{theorem}




\begin{algorithm}[t]
\caption{The C-GAIL algorithm}\label{alg:cap}
\begin{algorithmic}[1]
 \STATE {\bfseries Input:} Expert trajectory $\tau_E$ sampled from $\pi_E$, initial parameters $\theta_0$, and $\phi_0$ for generator and discriminator. 
  \REPEAT
\STATE Sample trajectory $\tau$ from $\pi_{\theta}$. 

\STATE Update discriminator parameters $\phi$ with gradient from,\\
$\hat{\mathbb{E}}_\tau \left[\log D(s,a) - \left(\frac{k}{2}(D(s,a) - \frac{1}{2}\right)^2 \right]  + \hat{\mathbb{E}}_{\tau_E} \left[\log(1-D(s,a))- \left(\frac{k}{2}(D(s,a) - \frac{1}{2}\right)^2 \right]$
\\ \tp{check brackets here}
\STATE Update policy parameters $\theta$ with $V_\pi (D, \pi)$ in Eq. \ref{obj1}

\UNTIL{Stopping criteria reached}
% \UNTIL{$\operatorname{maxiter}$ reaches}
\end{algorithmic}
% \vspace{0.05in}
\end{algorithm}



\section{A Practical Method to Stabilize GAIL} \label{sec:loss}
In this section, we extend our controller from the ``one-step'' setting back to the general setting and instantiate our controller as a regularization term on the original GAIL loss function. This results in our proposed variant C-GAIL; a  method to stabilize the training process of GAIL.

%Motivated by the above analysis, we further extend our controller to be incorporated into the objective functions of GAIL. The controllers in Eq. (\ref{eq_u2}) are designed to make GAIL's training dynamic converge to the desired state. 
Since the controllers in Eq. (\ref{eq_u2}) are defined in the dynamical system setting, we need to integrate these with respect to time, in order to recover an objective function that can be practically optimized by a GAIL algorithm.
%We note that whilst our theoretical guarantees may not hold in the pragmatic version, this follows a precedent for designing stable GAN variants. For example, \citet{xu2020understanding, luo2023stabilizing} proposed their controller in the simplified linear Dirac-GAN \citep{mescheder2018training} model, which guided them to design practical algorithms that perform well empirically despite falling outside of the simplified setting.\junz{looks like a straightforward adaptation from GAN to GAIL? what's the key difference/challenges?}
% particularly interested in reflecting controllers in loss functions. To do so, we take the integration of the dynamical system to get the controlled loss functions for the discriminator and generator. 
% Our controllers are designed for GAIL's training dynamic. However, we are particularly interested in reflecting controllers in loss functions. To do so, we take the integration of the dynamical system to get the controlled loss functions for the discriminator and generator. 
% \tj{we may need to explain the connection from simplified version to original setting}
% In practice, we incorporate our controller into the loss function in Eq.~ (\ref{obj1}) and empirically show the effectiveness of our C-GAIL. 
% In Section \ref{sec:controlller} we designed an ideal controller under a simplified setting. We now consider how this can be implemented in a practical algorithm through modification of the loss function in Eq.~ (\ref{obj1}).
Recalling that $V_D(D, \pi)$ and $V_\pi(D, \pi)$ are the original GAIL loss functions for the discriminator and policy (Eq.~(\ref{obj1})), we define $V_D'(D, \pi)$ and $V_\pi'(D, \pi)$ as modified loss functions with the integral of our controller applied, such that
\begin{equation*}
\begin{aligned}
     V_D'(D,\pi) &= V_D(D, \pi) - \mathbb{E}_{\pi, \pi_E}\left[\frac{k}{2}(D(s, a)-\frac{1}{2})^2\right], \\
      V_\pi' (D, \pi) &= V_\pi(D, \pi) + \mathbb{E}_{\pi, \pi_E} \left[\frac{\alpha}{2} \frac{\pi^2(a|s)}{\pi_E (a|s)}    + (c \log \frac{1}{2} + c\lambda \log \pi_E(a|s) + c\lambda - \alpha)\pi(a|s)\right].
      \end{aligned}
\end{equation*}
% $
%      V_D'(D,\pi)= V_D(D, \pi) - \mathbb{E}_{\pi, \pi_E}[\frac{k}{2}(D(s, a)-\frac{1}{2})^2]$ and $
%      V_\pi' (D, \pi) &= V_\pi(D, \pi) + \mathbb{E}_{\pi, \pi_E} [\frac{\alpha}{2} \frac{\pi^2(a|s)}{\pi_E (a|s)}    + (c \log \frac{1}{2} + c\lambda \log \pi_E(a|s) + c\lambda - \alpha)\pi(a|s)]$.
     % \jianfei{change $E$} 
Note that the training dynamics with these loss functions are identical to Eq.~(\ref{eqxu}-\ref{eq_u2}) with guaranteed stability under the `one-step' setting. 
% \tp{would be nice to break eqs onto separate lines if space allows}

% \tp{is it more intuitive to write $-k/2(D-1/2)^2$?}

% We denote $V_D(D, \pi)$ as the original loss function for the discriminator and $V_D'(D, \pi)$ as our controlled loss function, where 
% \begin{equation}
%      V_D'(D,\pi)= V_D(D, \pi) -\frac{k}{2}D^2(s, a) + \frac{k}{2} D(s, a)
% \end{equation}
% Similarly, we denote $V_\pi(D, \pi)$ as the original loss function for the discriminator and $V_\pi'(D, \pi)$ as our controlled loss function, where 
% \begin{align}
%     V_\pi' (D, \pi) &= V_\pi(D, \pi) \nonumber - (c \log \frac{1}{2} + c\lambda \log E - \alpha)\pi(a|s) \nonumber \\
%     &\quad +\frac{\alpha}{2E} \pi^2(a|s),
% \end{align}

While $V_D'(D,\pi)$ can be computed directly, the inclusion of $\pi_E$, the expert policy, in $V_\pi' (D, \pi)$ is problematic -- the very goal of the algorithm is to learn $\pi_E$, and we do not have access to it during training. Hence, in our practical implementations, we only use our modified loss $V_D'(D,\pi)$ to update the discriminator, but use the original unmodified policy objective $V_\pi (D, \pi)$  for the policy. In other words, we only add the controller to the discriminator objective $V_D(D,\pi)$. This approximation has no convergence guarantee, even in the one-step setting. Nevertheless, the control theory-motivated approach effectively stabilizes GAIL in practice, as we shall see in Sec.~\ref{Evaluation}. Intuitively, C-GAIL pushes the discriminator to its equilibrium at a faster speed by introducing a penalty controller centered at $\frac{1}{2}$. With proper selection of the hyperparameter $k$ (ablation study provided in Appendix \ref{appD}), the policy generator is able to train the discriminator at the same pace, leading GAIL's training to converge faster with a smaller range of oscillation, and match the expert distribution more closely.

Our C-GAIL algorithm is listed in Alg.~\ref{alg:cap}. It can be implemented by simply adding a regularization term to the discriminator loss. 
%, and the controlling effect would be automatically implemented with automatic differentiation. 
Hence, our method is also compatible with other variants of GAIL, by straightforwardly incorporating the regularization into their discriminator objective function. 
%Empirically we find that our algorithm is effective in GAIL variants such as GAIL-DAC. Evaluations follow in Section \ref{Evaluation}.

%\jianfei{should discuss why the practical algorithm can work, here or in sec. 6?}




% Note that the value of hyperparameters $k$ and $\alpha$ should be bounded by Assumption \ref{assumption}. 

% \tp{well we don't use $\alpha$ in the algorithm, so not sure how applicable the bounds are.}

% \tp{tj did you ever try plugging in the current GAIL policy inplace of E. glancing at it, eq 24 might end up reducing to something silly with that anyway.. worth adding some detail?}

% Notice that the value of hyperparameters $k$ and $\alpha$ should be bounded by assumption \ref{assumption}. Now we are concerning reflecting the new loss function into our algorithm. In practice, we are unaware of the expert policy for the generator's controller, so in the evaluation section, we only include the controller for the discriminator. In original GAIL, we sample $\tau$ and $\tau_E$ from policy $\pi$ and $\pi_E$ respectively and update the discriminator with function $\hat{\mathbb{E}}_\tau[\log D(s,a)] + \hat{\mathbb{E}}_{\tau_E}[\log (1-D(s,a))]$. As a result, we modify the discriminator update with our controller as shown in Algorithm \ref{alg:cap}.




% We emphasize that whilst our controller was designed for the simplified one environmental step version of vanilla GAIL, the C-GAIL algorithm does not necessarily offer the same theoretical stability guarantees. 
% Whilst our controller is designed for the simplified one environmental step version of vanilla GAIL, empirically we find that it is also effective in GAIL variants such as GAIL-DAC. Evaluations follow in Section \ref{Evaluation}.

% Even though our controller is designed for the simplified one environmental step version of vanilla GAIL, in practice we find out our controller is also applicable to other GAIL variants such as GAIL-DAC. We evaluate our controller on vanilla GAIL and GAIL-DAC in Section \ref{Evaluation}. Our method successfully speed up the rate of convergence and stabilize the training process. 


==> Styles/input/5-experiment.tex <==


\section{Evaluation} \label{Evaluation}


% \jianfei{you should have a place to also mention GAIL variants's formulation. maybe in Sec. 2.1 or Sec. 3, and claim that your algorithm is not limited to the original GAIL, but also applicable to GAIL variants. If your work is only applicable to original GAIL, its value will be quite limited. This makes a huge impact in assessing your paper. Make it clear.}

% This section evaluates the controlled loss function developed in Section \ref{control} 
This section evaluates the benefit of integrating the controller developed in Section \ref{control} with popular variants of GAIL. 
We test the algorithms on their ability to imitate an expert policy in simulated continuous control problems in MuJoCo \citep{todorov2012mujoco}.
% Since our proposal can be implemented as a modified objective function
Specifically, we consider applying our controller to two popular GAIL algorithms -- both the original `vanilla' GAIL \citep{ho2016generative} and also GAIL-DAC \citep{kostrikov2018discriminator}, a state-of-the-art variant which uses a discriminator-actor-critic (DAC) to improve sample efficiency and reduce the bias of the reward function.
% \junz{the integration and variants of GAIL were already discussed in Sec 4, don't go backward to re-duplicate. that makes the logic too complicated/confusing. re-organize the content to make the paper flows naturally forward... }
{Additionally, we include supplementary experiments compared with other GAIL variants such as  \citet{jena2021augmenting} and \citet{ xiao2019wasserstein} in appendix \ref{suppexp}.}

% For vanilla GAIL, we leverage the implementation provided by \citet{gleave2022imitation}, which provides widely-used baselines for imitation learning methods including BC, AIRL, vanilla GAIL, and dataset aggregation (DAgger) \citep{ross2011reduction}. 
% For GAIL-DAC, we extend the implementation from \citet{kostrikov2018discriminator}.
% , modify its objective function to accommodate our C-GAIL-DAC. 
% \tp{maybe add DAC implementation?} \tj{added a few sentences}
% For GAIL-DAC, we implement based on \citet{kostrikov2018discriminator}, and modify its objective function to accommodate our C-GAIL-DAC. \tp{maybe add DAC implementation?} \tj{added a few sentences}

% We evaluate and compare the speed of convergence and the performance of our controller GAIL comparing with naive GAIL and GAIL-DAC.


% In this section, we implement our designed controller in section \ref{sec:controlller} and evaluate its performance on different environments. Our experiments are based on the naive GAIL \citep{ho2016generative} and GAIL-DAC \citet{kostrikov2018discriminator}, which uses a discriminator-actor-critic (DAC) to improve the sample efficiency of GAIL and reduce the bias for the reward function. We also work under IMITATION framework \citep{gleave2022imitation}, which provides reliable baselines for imitation learning methods including BC,  AIRL, GAIL, and dataset aggregation (DAgger) \citep{ross2011reduction}, simulated on various MuJoCo environments \citep{todorov2012mujoco}. We evaluate and compare the speed of convergence and the performance of our controlled GAIL comparing with naive GAIL and GAIL-DAC.

% \begin{figure*}[h]
%     \centering
% \includegraphics[scale=0.253]{input/fig/distance_cheetah.pdf}
% \includegraphics[scale=0.253]{input/fig/distance_walker.pdf}
% \includegraphics[scale=0.253]{input/fig/distance_reacher.pdf}
% \includegraphics[scale=0.253]{input/fig/distance_ant.pdf}
% \includegraphics[scale=0.253]{input/fig/distance_hopper.pdf}
%     \caption{State Wasserstein distance over training between expert and learned policies (lower better). Our controlled variant matches the expert distribution more closely.}
%     % \caption{The state Wasserstein distance\(\downarrow\) over the number of gradient step updates with4ExpertDemostrations.}
%     \label{fig:distance}

% \end{figure*}

\begin{figure}[t]  
    \centering
    % \vspace{-0.1in}
\begin{minipage}{0.327\linewidth}
	\centering
 {\footnotesize Half-Cheetah}
	\includegraphics[width=\linewidth]{Styles/input/fig/distance_cheetah.pdf}
\end{minipage} 
\begin{minipage}{0.327\linewidth}
	\centering
 {\footnotesize Walker}
	\includegraphics[width=\linewidth]{Styles/input/fig/distance_walker.pdf}
\end{minipage} 
\begin{minipage}{0.327\linewidth}
	\centering
 {\footnotesize Reacher}
	\includegraphics[width=\linewidth]{Styles/input/fig/distance_reacher.pdf}
\end{minipage} \\


\begin{minipage}{0.327\linewidth}
	\centering
     {\footnotesize Ant}
	\includegraphics[width=\linewidth]{Styles/input/fig/distance_ant.pdf}
\end{minipage} 
\begin{minipage}{0.327\linewidth}
	\centering
 {\footnotesize Hopper}
	\includegraphics[width=\linewidth]{Styles/input/fig/distance_hopper.pdf}
\end{minipage} 
 \\
 % \vspace{-0.1in}
 \caption{State Wasserstein distance (lower is better) between expert and learned policies, over number of gradient step updates. Our controlled variant matches the expert distribution more closely.}
    % \caption{The state Wasserstein distance\(\downarrow\) over the number of gradient step updates with4ExpertDemostrations.}
    \label{fig:distance}
\vspace{-0.1in}
\end{figure}


% \begin{figure}[h!]
% \centering
% \begin{minipage}{0.327\linewidth}
% 	\centering
%         {\footnotesize Half-Cheetah} 
% 	\includegraphics[width=\linewidth,height=2.5cm]{input/fig/Half-Cheetah4ExpertDemostrations.pdf}
% \end{minipage} 
% \begin{minipage}{0.327\linewidth}
% 	\centering
% 	\includegraphics[width=\linewidth]{Styles/input/fig/Half-convergence.pdf}
% \end{minipage} 
% \begin{minipage}{0.327\linewidth}
% 	\centering

% 	\includegraphics[width=\linewidth]{Styles/input/fig/distance_cheetah.pdf}
% \end{minipage} \\


% \begin{minipage}{0.327\linewidth}
% 	\centering
%         {\footnotesize Ant} 
% 	\includegraphics[width=\linewidth,height=2.5cm]{Styles/input/fig/Ant4ExpertDemostrations.pdf}
% \end{minipage} 
% \begin{minipage}{0.327\linewidth}
% 	\centering
% 	\includegraphics[width=\linewidth]{Styles/input/fig/Ant-convergence.pdf}
% \end{minipage} 
% \begin{minipage}{0.327\linewidth}
% 	\centering
% 	\includegraphics[width=\linewidth]{Styles/input/fig/distance_ant.pdf}
% \end{minipage} \\


% \begin{minipage}{0.327\linewidth}
% 	\centering
%         {\footnotesize Reacher} 
% 	\includegraphics[width=\linewidth,height=2.5cm]{Styles/input/fig/Reacher4ExpertDemostrations.pdf}
% \end{minipage} 
% \begin{minipage}{0.327\linewidth}
% 	\centering
% 	\includegraphics[width=\linewidth]{Styles/input/fig/Reacher-convergence.pdf}
% \end{minipage} 
% \begin{minipage}{0.327\linewidth}
% 	\centering
% 	\includegraphics[width=\linewidth]{Styles/input/fig/distance_reacher.pdf}
% \end{minipage} \\

% \begin{minipage}{0.327\linewidth}
% 	\centering
%         {\footnotesize Walker} 
% 	\includegraphics[width=\linewidth,height=2.5cm]{Styles/input/fig/Walker2d4ExpertDemostrations.pdf}
% \end{minipage} 
% \begin{minipage}{0.327\linewidth}
% 	\centering
% 	\includegraphics[width=\linewidth]{Styles/input/fig/Walker-convergence.pdf}
% \end{minipage} 
% \begin{minipage}{0.327\linewidth}
% 	\centering
% 	\includegraphics[width=\linewidth]{Styles/input/fig/distance_walker.pdf}
% \end{minipage} \\

% \begin{minipage}{0.327\linewidth}
% 	\centering
%         {\footnotesize Hopper} 
% 	\includegraphics[width=\linewidth,height=2.5cm]{Styles/input/fig/Hopper4ExpertDemostrations.pdf}
% \end{minipage} 
% \begin{minipage}{0.327\linewidth}
% 	\centering
% 	\includegraphics[width=\linewidth]{Styles/input/fig/Hopper-convergence.pdf}
% \end{minipage} 
% \begin{minipage}{0.327\linewidth}
% 	\centering
% 	\includegraphics[width=\linewidth]{Styles/input/fig/distance_hopper.pdf}
% \end{minipage} 


% \end{figure}

\subsection{Experimental Setup} \label{settings}
We incorporate our controller in vanilla GAIL and GAIL-DAC, naming our controlled variants C-GAIL and C-GAIL-DAC. 
We leverage the implementations of \citet{gleave2022imitation} (vanilla GAIL) and \citet{kostrikov2018discriminator} (GAIL-DAC). \citet{gleave2022imitation} also provide other common imitation learning frameworks -- BC, AIRL, and dataset aggregation (DAgger) \citep{ross2011reduction} -- which we also compare to.  

% For vanilla GAIL, we leverage the implementation provided by \citet{gleave2022imitation}, which provides widely-used baselines for imitation learning methods including BC, AIRL, vanilla GAIL, and dataset aggregation (DAgger) \citep{ross2011reduction}. 
% For GAIL-DAC, we extend the implementation from \citet{kostrikov2018discriminator}.
% \vspace{-0.2in}
For C-GAIL-DAC, we test five MuJuCo environments: Half-Cheetah, Ant, Hopper, Reacher and Walker 2D. Our experiments follow the same settings as \citet{kostrikov2018discriminator}. The discriminator architecture has a two-layer MLP with 100 hidden units and tanh activations. The networks are optimized using Adam with a learning rate of $10^{-3}$, decayed by $0.5$ every $10^5$ gradient steps. We vary the number of provided expert demonstrations: $\{4, 7, 11, 15, 18\}$, though unless stated we report results using four demonstrations. We assess the normalized return over training for GAIL-DAC and C-GAIL-DAC to evaluate their speed of convergence and stability, reporting the mean and standard deviation over five random seeds.
The normalization is done with 0 set to a random policy's return and 1 to the expert policy return. 

In addition to recovering the expert's return, we are also interested in how closely our policy generator's and the expert's \textit{state distribution} are matched, for which we use the \textbf{state Wasserstein} \citep{pearce2023imitating}. This requires samples from two distributions, collected by rolling out the expert and learned policy for 100 trajectories each. We then use the POT library’s `emd2' function \citep{flamary2021pot} to compute the Wasserstein distance, using the L2 cost function with a uniform weighting across samples.

To evaluate C-GAIL, we follow the experimental protocol from \citet{gleave2022imitation}, both for GAIL and other imitation learning baselines. These are evaluated on Ant, Hopper, Swimmer, Half-Cheetah and Walker 2D. For C-GAIL, we change only the loss and all other GAIL settings are held constant. We assess performance in terms of the normalized return. We use this set up to ablate the controller strength hyperparameter of C-GAIL (Appendix \ref{appD}), varying $k \in \{0.1, 1, 10\}$ (ablation study of $\alpha$ is not included since our algorithm only involves controller for the discriminator in practice). Our experiments are conducted on a single NVIDIA GeForce GTX TITAN X. 

% For comparing GAIL and C-GAIL, we follow the experimental protocol from \citet{gleave2022imitation}, both for GAIL and other imitation learning baselines, evaluating on Ant, Hopper, Swimmer, Half-Cheetah and Walker 2D. For C-GAIL, we changes only the loss and all settings are otherwise held constant. We compare the performance of GAIL and C-GAIL in terms of the normalized return for various values of hyperparameter $k$ of our controller, including $\{0.1, 1, 10\}.$ to show the effectiveness of our controller. \tp{seems unbalnaced to describe so much more of GAIL-DAC, listing envs, learning rates etc. Should we do that for vanilla GAIL?} \tj{added a few sentences}

% for GAIL, BC, AIRL, and DAgger baselines. We modify the loss function of GAIL as in section \ref{sec:loss} and evaluate our controlled GAIL with the same settings as in GAIL. 

% We implement our controlled GAIL on both GAIL-DAC and naive GAIL. For GAIL-DAC, we work under 5 MuJuCo environments including Half-Cheetah, Ant, Hopper, Reacher and Walker 2d. Our experiments follows excatly the same setting as \citep{kostrikov2018discriminator}. The discriminator architecture has a 2 layer MLP with 100 hidden units and tanh activations. The networks are trained with Adam optimizer with a learning rate initiated at $10^{-3}$ and decayed by $0.5$ every $10^5$ gradient steps. We compare under 4 numbers of expert demonstrations. For each environment, we compute and compare the normalized return with respect to the number of gradient step for GAIL-DAC and controlled GAIL-DAC to evaluate their speed of convergence and stability. We take five random seeds per trail and we compute the average and standard deviation for the five seeds. 

% We replicate the exact experimental setup as reported in \citet{gleave2022imitation} for GAIL, BC, AIRL, and DAgger baselines. We modify the loss function of GAIL as in section \ref{sec:loss} and evaluate our controlled GAIL with the same settings as in GAIL. 







% \begin{figure*}[h]
%     \centering
%     \includegraphics[scale=0.22]{input/fig/Half-convergence.pdf}
%     \includegraphics[scale=0.22]{input/fig/Walker-convergence.pdf}
%     \includegraphics[scale=0.22]{input/fig/Reacher-convergence.pdf}
%     \includegraphics[scale=0.22]{input/fig/Ant-convergence.pdf}
%     \includegraphics[scale=0.22]{input/fig/Hopper-convergence.pdf}
    
%     \caption{Number of gradient step updates required to reach $95\%$ of the max-return for various number of trajectories on MuJoCo environments averaged over five random seeds}
%     \label{fig:dac-converge}
% \end{figure*}

\begin{figure}[b]  
    \centering
    \vspace{-0.1in}
\begin{minipage}{0.327\linewidth}
	\centering
 {\footnotesize Ant}
	\includegraphics[width=\linewidth]{Styles/input/fig/Ant-convergence.pdf}
\end{minipage} 
\begin{minipage}{0.327\linewidth}
	\centering
 {\footnotesize Walker}
	\includegraphics[width=\linewidth]{Styles/input/fig/Walker-convergence.pdf}
\end{minipage} 
\begin{minipage}{0.327\linewidth}
	\centering
 {\footnotesize Reacher}
	\includegraphics[width=\linewidth]{Styles/input/fig/Reacher-convergence.pdf}
\end{minipage} \\


\begin{minipage}{0.327\linewidth}
	\centering
     {\footnotesize Half-Cheetah}
	\includegraphics[width=\linewidth]{Styles/input/fig/Half-convergence.pdf}
\end{minipage} 
\begin{minipage}{0.327\linewidth}
	\centering
 {\footnotesize Hopper}
	\includegraphics[width=\linewidth]{Styles/input/fig/Hopper-convergence.pdf}
\end{minipage} 
 \\
 % \vspace{-0.1in}
 \caption{Number of gradient step updates (in millions) required to reach $95\%$ of the max-return for various numbers of expert trajectories on MuJoCo environments averaged over five random seeds.}
 \label{fig:dac-converge}
\end{figure}


\iffalse
\begin{figure}[h!]
    \centering
    \small Half-Cheetah\\
    \small Mean Return \hspace{0.9in} Wasserstein \\
    \includegraphics[width=0.49\columnwidth]{input/fig/Half-Cheetah,4ExpertDemostrations.pdf}
    \includegraphics[width=0.49\columnwidth]{input/fig/distance_cheetah.pdf}

    \small Walker 2D \\
    \includegraphics[width=0.49\columnwidth]{input/fig/Walker2d,4ExpertDemostrations.pdf}
    \includegraphics[width=0.49\columnwidth]{input/fig/distance_walker.pdf}

    \small Reacher \\
    \includegraphics[width=0.49\columnwidth]{input/fig/Reacher,4ExpertDemostrations.pdf}
    \includegraphics[width=0.49\columnwidth]{input/fig/distance_reacher.pdf}

    \small Ant \\
    \includegraphics[width=0.49\columnwidth]{input/fig/Ant,4ExpertDemostrations.pdf}
    \includegraphics[width=0.49\columnwidth]{input/fig/distance_ant.pdf}

    \small Hopper\\
    \includegraphics[width=0.49\columnwidth]{input/fig/Hopper,4ExpertDemostrations.pdf}
    \includegraphics[width=0.49\columnwidth]{input/fig/distance_hopper.pdf}
    
    \caption{Possible new fig? If go with this, make style of each the same -- background color, line colors, aspect ratio,  font size (probably match wasserstein which suits the taller ratio better). Also only need legend in one plot, title per environment can be shared and added across both. No need for individ titles.}
    \label{fig:dac-return-combo}
\end{figure}
\fi



\begin{table*}[h!]  
\caption{Mean and standard deviation for returns of various IL algorithms and environments}
    \centering
    \begin{tabular}{c|c|c|c|c|c}
    \hline
         & Ant & Half Cheetah & Hopper& Swimmer & Walker2d \\
         \hline

        Random & $-349 \pm 31$ & $-293 \pm 36$ & $-53 \pm 62$&  $3 \pm 8$& $-18 \pm 75$\\
       Expert  & 
        $2408 \pm 110$ & $3465 \pm 162$ & $2631  \pm  19$&$298 \pm 1$ & $2631 \pm 112$ \\

        
       Controlled GAIL  & $2411 \pm 21$& $3435 \pm 50$ & $2636 \pm 8$& $298 \pm 0$ & $2633 \pm 12$\\
       
       GAIL &  $2087 \pm 187$ & $3293 \pm 239$ & $2579 \pm 85$ & $295 \pm 3$ & $2589 \pm 121$ \\

       
       BC & $1937 \pm 227$ &  $ 3465 \pm 151$& $ 2830 \pm 265 $  & $ 298 \pm 1$ & $ 2672 \pm 95$\\

        AIRL & $-121 \pm 28$&  $1837 \pm 218$  & $2536 \pm 142$ & $ 269 \pm 8$& $1329 \pm 134$\\

        DAgger & $3027 \pm 187$& $1693 \pm 74$&$2751 \pm 11$& $ 344 \pm 2$& $2174 \pm 132$\\
       
    \hline
    \end{tabular}
    \label{tab:return}
    \vspace{-0.1in}
\end{table*}



\subsection{Results}

% \textbf{Controlled GAIL-DAC} 
We compare GAIL-DAC to C-GAIL-DAC in Figure \ref{fig:dac-return} (return),  \ref{fig:distance} (state Wasserstein), and \ref{fig:dac-converge} (convergence speed). 
Figure \ref{fig:dac-return} shows that C-GAIL-DAC speeds up the rate of convergence and reduces the oscillation in the return training curves across all environments. For instance, on Hopper, C-GAIL-DAC converges 5x faster than GAIL-DAC with less oscillations. On Reacher, the return of GAIL-DAC continues to spike even after matching the expert return, but this does not happen with C-GAIL-DAC. On Walker 2D, the return of GAIL-DAC oscillates throughout training, whereas our method achieves a higher return at has reduced the range of oscillation by more than 3 times. For Half-Cheetah, our method converges 2x faster than GAIL-DAC. For Ant environment, C-GAIL-DAC reduces the range of oscillations by around 10x. 
% \tp{not sure going through each env one by one is particularly needed -- could shorten this by summarizing trends for all envs and picking out 1-2 specific remarks.}

In addition to matching the expert's return faster and with more stability, Figure \ref{fig:distance} shows that C-GAIL-DAC also more closely matches the expert's state distribution than GAIL-DAC, with the difference persisting even towards the end of training for various numbers of expert trajectories. Toward the end of training, the state Wasserstein for C-GAIL-DAC is more than two times smaller than the state Wasserstein for GAIL-DAC on all five environments.

Figure \ref{fig:dac-converge} shows that these improvements hold for differing numbers of provided demonstrations. It plots the number of gradient steps for GAIL-DAC and C-GAIL-DAC to reach $95\%$ of the max-return for vaious numbers of expert demonstrations. Our method is able to converge faster than GAIL-DAC regardless of the number of demonstrations. 
% For example, in Hopper our method converges 10x faster with four expert demonstrations.
% We record the number of gradient step updates for GAIL-DAC and our method to reach $95\%$ of their expert's return with respect to different number of expert demonstrations in Figure \ref{fig:dac-converge}. Our method is able to converge much more faster than GAIL-DAC regardless of the number of demonstrations given. Furthermore, for Hopper, our method is able to converge 10x faster with 4 expert demonstrations.


% Note that the low spikes seen in several environments are due to ... \tp{explain here if don't fix}

% \tp{todo}
% As shown in Figure \ref{fig:distance}, the state Wasserstein of our C-GAIL-DAC has a large distance shift at the beginning stage of training, which accords with the fact that our method is able to converge faster. Additionally, the state Wasserstein for C-GAIL-DAC is 2.5X smaller than GAIL-DAC and approaches to 0 as the number of gradient step updates increases, which indicates that our C-GAIL-DAC has a smaller range of oscillation. 

% \textbf{Controlled GAIL-DAC} Our controlled GAIL-DAC is able to speed up the rate of convergence and reduce the radius of oscillation in experiments. As shown in figure \ref{fig:dac-return}, we compare the normalized return of our controlled GAIL-DAC to original GAIL-DAC averaged over five random seeds on various MuJuCo tasks. Specifically, on Hopper environment, our controlled GAIL-DAC converge 5x faster than original GAIL-DAC and significantly reduce the radius of convergence on the early stage of training. On Reacher environment, GAIL-DAC has sudden drop in the middle of training process and a large range of oscillation, and our controlled GAIL-DAC reduce the range of oscillation by more than 8 times. On Walker2d, GAIL-DAC has a giant range of oscillation throughout the training process, whereas our method achieves a higher return at has reduced the range of oscillation by more than 3 times. For Half-Cheetah, our method converges 2x faster than GAIL-DAC. For Ant environment, our method reduce the range of oscillation by around 10x throughout the training process.


 


% Moreover, we record the number of gradient step updates for GAIL-DAC and our method to reach $95\%$ of their max-return with respect to different number of expert demonstrations in Figure \ref{fig:dac-converge}. Our method is able to converge much more faster than GAIL-DAC regardless of the number of demonstrations given. Furthermore, for Hopper, our method is able to converge 10x faster with 4 expert demonstrations. 





\textbf{Hyperparameter sensitivity.} We evaluate the sensitivity to the controller's hyperparameter $k$ using vanilla GAIL. 
Figure \ref{fig:return} (Appendix \ref{appD}) plots normalized returns. For some environments, minor gains can be found by tuning this hyperparameter, though in general for all values tested, the return curves of C-GAIL approach the expert policy's return earlier and with less oscillations than GAIL. This is an important result as it shows that our regularizer can easily be applied by practitioners without the need for a fine-grained hyperparameter sweep.

% \textbf{Hyperparameter sensitivity} We evaluate and compare the performance of our controlled GAIL with original GAIL for different hyperparameters of controllers with $k=0.1$, $k=1$, and $k=10$. We normalize the return on the y-axis such that 0 refers to the random policy return and 1 refers to the expert policy return.  As shown in figure \ref{fig:return}, the training curves of our controlled GAIL approaches to the expert policy at an earlier stage than GAIL and have a smaller range of osculations around the expert policy return. 

\textbf{Other imitation learning methods.}
Table \ref{tab:return} benchmarks C-GAIL against other imitation learning methods, including BC, AIRL, and DAgger, some of which have quite different requirements to the GAIL framework.
% As such, whilst this comparison is a broader evaluation of the GAIL framework, 
The table shows that C-GAIL is competitive with many other paradigms, and in consistently offers the lowest variance between runs of any method. Moreover, we include supplementary experiments compared with \citet{jena2021augmenting} and \citet{ xiao2019wasserstein} in appendix \ref{suppexp}.




% We then compare our controlled GAIL with other IL methods, including BC, AIRL, and DAgger. From table \ref{tab:return} (in Appendix \ref{appC}), we can see that in each environment, the mean returns for controlled GAIL are closer to expert policy returns, and the standard deviations for controlled GAIL are smaller than other IL methods. 

% \textbf{State Wasserstein} \tj{Tim you can also reference to your paper if you wish and introduce a little bit on State Wasserstein} We measure the state wassertein between two consecutive policy generators over the number of gradient step updates. Specifically, we sample 100 trajectories per distribution and ... \tj{Can you fill in the description for this one? Maybe also add an equation for how the distance is measured}. As shown in Figure \ref{fig:distance}, the state Wasserstein of our C-GAIL-DAC has a large distance shift at the beginning stage of training, which accords with the fact that our method is able to converge faster. Additionally, the state Wasserstein for C-GAIL-DAC is 2.5X smaller than GAIL-DAC and approaches to 0 as the number of gradient step updates increases, which indicates that our C-GAIL-DAC has a smaller range of oscillation. 



==> Styles/input/6-discussion.tex <==



\section{Discussion \& Conclusion} \label{discussion}
This work helped understand and address the issue of training instability in GAIL using the lens of control theory. This advances recent findings showing its effectiveness in other adversarial learning frameworks.
% , which has recently proven effective when applied to other adversarial learning frameworks. 
We formulated GAIL's training as a dynamical system and designed a controller that stabilizes it at the desired state, encouraging convergence to this point. We showed theoretically that our controlled system achieves asymptotic stability under a ``one-step'' setting. We proposed a practical realization of this named C-GAIL, which reaches expert returns both faster and with less oscillation than the uncontrolled variants, and also matches their state distribution more closely.

% In this work, 1) we formally establish the issue of unstable training for GAIL with control theory. 2) We formulate GAIL's training as a dynamical system and design a controller to stabilize and converge this dynamical system to the desired equilibrium. 3) Our controlled system achieves asymptotic stability in theory and successfully speeds up and stabilizes the training process of GAIL in experiments.


Whilst our controller theoretically converges to the desired state, and empirically stabilizes training, we recognize several limitations of our work. 
% As an imitation learning method, is cannot exceed the return of the expert demonstrator. 
In our description of GAIL training as a continuous dynamical system, we do not account for the updating of generator and discriminator being discrete as in practice. In our practical implementation of the controller, we only apply the portion of the loss function acting on the discriminator, since the generator portion requires knowing the likelihood of an action under the expert policy (which is precisely what we aim to learn!).
We leave it to future work to explore whether estimating the expert policy and incorporating a controller for the policy generator brings benefit. 

% \textbf{Future Work.}
% Even though our controller theoretically and empirically converges and stabilizes the return of GAIL to expert policy return, we are looking forward to maximizing return in reinforcement learning. Our controller may restrict the growth of generator policy return by forcing it to converge to expert policy return. In addition, when transforming GAIL's training to a dynamical system in section \ref{sec:dynamic}, we consider the training process of GAIL as a continuous dynamical system, whereas the alternative updating between the generator and the discriminator should be discrete in practice. Furthermore, we implement our controller only on the loss function of the discriminator for our evaluation since we are unaware of the expert policy included in the controller for the policy generator. However, future work can explore estimating the expert policy with numerical methods and add the controller for the policy generator as well. \\


% \tp{never really know what they want here, feel free}

% the same social-ethical problem as other imitation learning methods, such as the potential invasion of privacy when collecting expert data and learning unwanted or unlawful behaviors from expert data. Additionally, when an agent performs an action that may be harmful, the legal responsibility is still unclear. 
% This work confronts the same social-ethical problem as other imitation learning methods, such as the potential invasion of privacy when collecting expert data and learning unwanted or unlawful behaviors from expert data. Additionally, when an agent performs an action that may be harmful, the legal responsibility is still unclear. 





